Observational Indistinguishability and Integrity Blind Regions in Hybrid Quantum-Classical Workflows

We present a claim-relative evidence/reference framework for hybrid quantum-classical workflow integrity. Observational indistinguishability yields structural blind regions, distinct from finite-batch statistical misses. Within the declared lattice, a trusted same-batch scalar $R_0$ suffices for conclusion integrity, aggregate $M_0$ for aggregate plus conclusion integrity, and item-aligned binding for item identity. In 3,600 label interventions, feature/prediction views realize exact label-path invariance; all 764 geometry-aligned aggregate-blind rows equal their paired-clean responses, giving zero attack-only increment. For statistical response, the geometry-aligned construction detects 343/2,700 conclusion-changing ($\tau \to 0^+$) label interventions with the conformal rule and 1,183/2,700 with the uncorrected union; the original frozen same-item geometry yields 11/2,617 and 43/2,617, respectively. The executed conformal clean false-action rates are 0.048--0.059 descriptively; its finite-sample guarantee requires exchangeability, which the overlapping-draw design violates. The cluster-preserving adaptive stress test (Gate A) reduces response versus matched controls in 25--40 of 40 environment/split cells while retaining conclusion changes. A bounded 165-design-cell ideal-statevector and finite-shot-emulation branch directly instantiates semantic, estimated and observed kernel transitions. The fixed equal-weight design estimates neither deployment prevalence nor QPU, provider or deployed-service assurance.

==> tables/m_adversarial.tex <==
\begin{table*}[!tbp]
\caption{Gate A: executed drift mechanisms (matched controls, frozen strengths) against their adaptive cluster-preserving variants (class F5), 600 observations per row pooled over the eight environments. Detection uses the conformal family rule in $\mathcal I_X$ and $\mathcal I_{XF}$; material is the fraction with changed balanced accuracy; served is the number of undetected materially altered audit results served by P2 in $\mathcal I_{XF}$ over material rows. The attacker leaves clustered entries untouched and perturbs the remaining 32\% on average.}
\label{tab:adversarial}
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lrrrrrrrrr@{}}
\toprule
 & & \multicolumn{4}{c}{Executed mechanism (control)} & \multicolumn{4}{c}{Cluster-preserving (adaptive, F5)} \\
\cmidrule(lr){3-6}\cmidrule(lr){7-10}
Mechanism & Strength & Det.\ $\mathcal I_X$ & Det.\ $\mathcal I_{XF}$ & Material & Served P2 & Det.\ $\mathcal I_X$ & Det.\ $\mathcal I_{XF}$ & Material & Served P2 \\
\midrule
Mean shift & 0.02 & 1.00 & 0.97 & 0.33 & 4/197 & 0.01 & 0.06 & 0.29 & 155/174 \\
Mean shift & 0.05 & 1.00 & 1.00 & 0.46 & 0/275 & 0.08 & 0.24 & 0.40 & 151/237 \\
Mean shift & 0.10 & 1.00 & 1.00 & 0.59 & 0/355 & 0.34 & 0.48 & 0.54 & 139/322 \\
Mean shift & 0.25 & -- & -- & -- & -- & 0.79 & 0.80 & 0.69 & 65/411 \\
Mean shift & 0.50 & -- & -- & -- & -- & 0.89 & 0.90 & 0.76 & 33/454 \\
\addlinespace[1pt]
Scaling drift & 0.02 & 0.99 & 0.96 & 0.48 & 2/290 & 0.05 & 0.23 & 0.40 & 131/241 \\
Scaling drift & 0.05 & 1.00 & 0.99 & 0.57 & 0/345 & 0.35 & 0.47 & 0.52 & 107/313 \\
Scaling drift & 0.10 & 1.00 & 1.00 & 0.64 & 0/386 & 0.56 & 0.66 & 0.58 & 76/350 \\
Scaling drift & 0.25 & -- & -- & -- & -- & 0.76 & 0.79 & 0.72 & 61/431 \\
Scaling drift & 0.50 & -- & -- & -- & -- & 0.88 & 0.88 & 0.81 & 41/485 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\end{table*}


==> tables/m_policy.tex <==
\begin{table}[!t]
\caption{Offline decisions on frozen observations at the structural-sensitivity endpoint $|\Delta_R|>0$ (7,008 materially altered audit results among 10,800 interventions). P1: union; P2: conformal, risk-tolerant; P3: sensor-coverage-complete relative to declared evidence dimensions and abstaining on missing coverage. FPR is estimated on 12,000 clean draws from evaluation pools disjoint from the calibration pools; resampled draws within a pool may overlap. The starred row instead reports an exact-zero invariant check on 1,200 rows and is not the same estimand. Benign is interruption of the same 1,200 near-null synthetic controls. Served: undetected materially altered audit results served, not malicious network events. Blind: structurally indistinguishable material rows.}
\label{tab:policy}
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}llrrrrr@{}}
\toprule
Regime & Policy & FPR/check & Benign & Served & Contain. & Blind \\
\midrule
$\mathcal I_X$ & P1 union & 0.125 & 0.76 & 4,429 & 0.37 & 2,617 \\
$\mathcal I_X$ & P2 conf. & 0.056 & 0.55 & 4,496 & 0.36 & 2,617 \\
$\mathcal I_X$ & P3 abst. & 1.000 & 1.00 & 0 & 1.00 & 2,617 \\
\addlinespace[1pt]
$\mathcal I_{XF}$ & P1 union & 0.203 & 0.76 & 4,231 & 0.40 & 2,617 \\
$\mathcal I_{XF}$ & P2 conf. & 0.058 & 0.52 & 4,365 & 0.38 & 2,617 \\
$\mathcal I_{XF}$ & P3 abst. & 1.000 & 1.00 & 0 & 1.00 & 2,617 \\
\addlinespace[1pt]
$\mathcal I_{Y_m}$ & P1 union & 0.048 & 0.00 & 7,008 & 0.00 & 5,450 \\
$\mathcal I_{Y_m}$ & P2 conf. & 0.048 & 0.00 & 7,008 & 0.00 & 5,450 \\
$\mathcal I_{Y_m}$ & P3 abst. & 1.000 & 1.00 & 0 & 1.00 & 5,450 \\
\addlinespace[1pt]
$\mathcal I_{XFY}$ & P1 union & 0.259 & 0.76 & 4,180 & 0.40 & 0 \\
$\mathcal I_{XFY}$ & P2 conf. & 0.053 & 0.49 & 4,390 & 0.37 & 0 \\
\addlinespace[1pt]
$\mathcal I_{XFY}^{\star}$ & P2/P3 (exact) & 0.000 & 0.52 & 0 & 1.00 & 0 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/m_v137_adversarial.tex <==
\begin{table*}[!tbp]
\caption{Gate A after the JSD correction: the same executed drift controls and cluster-preserving variants, 600 observations per row. Detection is the conformal-family response; materiality and predictions are unchanged. Served is P2 in $\mathcal I_{XF}$ among material rows. The construction reduces response against the declared fingerprint; it is not universal evasion.}
\label{tab:adversarial}
\centering\scriptsize\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lrrrrrrrrr@{}}
\toprule
 & & \multicolumn{4}{c}{Executed mechanism (control)} & \multicolumn{4}{c}{Cluster-preserving (adaptive, F5)} \\
\cmidrule(lr){3-6}\cmidrule(lr){7-10}
Mechanism & Strength & Det. $\mathcal I_X$ & Det. $\mathcal I_{XF}$ & Material & Served P2 & Det. $\mathcal I_X$ & Det. $\mathcal I_{XF}$ & Material & Served P2 \\
\midrule
Mean shift & 0.02 & 1.00 & 0.97 & 0.33 & 4/197 & 0.01 & 0.05 & 0.29 & 157/174 \\
Mean shift & 0.05 & 1.00 & 1.00 & 0.46 & 0/275 & 0.08 & 0.23 & 0.40 & 156/237 \\
Mean shift & 0.10 & 1.00 & 1.00 & 0.59 & 0/355 & 0.36 & 0.50 & 0.54 & 133/322 \\
Mean shift & 0.25 & -- & -- & -- & -- & 0.81 & 0.83 & 0.69 & 52/411 \\
Mean shift & 0.50 & -- & -- & -- & -- & 0.88 & 0.90 & 0.76 & 35/454 \\
\addlinespace[1pt]
Scaling drift & 0.02 & 0.99 & 0.96 & 0.48 & 2/290 & 0.05 & 0.23 & 0.40 & 131/241 \\
Scaling drift & 0.05 & 1.00 & 0.98 & 0.57 & 3/345 & 0.29 & 0.42 & 0.52 & 104/313 \\
Scaling drift & 0.10 & 1.00 & 1.00 & 0.64 & 0/386 & 0.57 & 0.65 & 0.58 & 74/350 \\
Scaling drift & 0.25 & -- & -- & -- & -- & 0.75 & 0.80 & 0.72 & 53/431 \\
Scaling drift & 0.50 & -- & -- & -- & -- & 0.88 & 0.89 & 0.81 & 43/485 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_adaptive_strength_profile.tex <==
\begin{table*}[!tbp]
\caption{Adaptive F5 profile by nominal strength, derived without rerunning any experiment. Material is changed balanced accuracy at the structural-sensitivity endpoint. Detection is the conformal family firing rate over all 600 rows; served is the P2 fraction among material rows. The first three strengths have matched executed controls; 0.25 and 0.50 are the preregistered extended adaptive grid.}
\label{tab:s-adaptive-strength-profile}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
 & & & \multicolumn{3}{c}{Detection, all rows} & \multicolumn{3}{c}{Material served by P2} \\
\cmidrule(lr){4-6}\cmidrule(lr){7-9}
Mechanism & Strength & Material & $\mathcal I_X$ & $\mathcal I_{XF}$ & $\mathcal I_{XFY}$ & $\mathcal I_X$ & $\mathcal I_{XF}$ & $\mathcal I_{XFY}$ \\
\midrule
Mean shift & 0.02 & 174/600 & 0.01 & 0.06 & 0.06 & 0.99 & 0.89 & 0.90 \\
Mean shift & 0.05 & 237/600 & 0.08 & 0.24 & 0.22 & 0.91 & 0.64 & 0.67 \\
Mean shift & 0.10 & 322/600 & 0.34 & 0.48 & 0.45 & 0.63 & 0.43 & 0.46 \\
Mean shift & 0.25 & 411/600 & 0.79 & 0.80 & 0.79 & 0.17 & 0.16 & 0.16 \\
Mean shift & 0.50 & 454/600 & 0.89 & 0.90 & 0.89 & 0.08 & 0.07 & 0.08 \\
Scaling drift & 0.02 & 241/600 & 0.05 & 0.23 & 0.22 & 0.89 & 0.54 & 0.55 \\
Scaling drift & 0.05 & 313/600 & 0.35 & 0.47 & 0.45 & 0.57 & 0.34 & 0.36 \\
Scaling drift & 0.10 & 350/600 & 0.56 & 0.66 & 0.65 & 0.34 & 0.22 & 0.22 \\
Scaling drift & 0.25 & 431/600 & 0.76 & 0.79 & 0.77 & 0.16 & 0.14 & 0.16 \\
Scaling drift & 0.50 & 485/600 & 0.88 & 0.88 & 0.86 & 0.10 & 0.08 & 0.10 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_adversarial_branch.tex <==
\begin{table*}[!tbp]
\caption{Gate A: detection of the adaptive variants under the conformal rule by branch (classical SVC on standardized features; fidelity kernels on features scaled to $[0,2\pi]$). The cluster rule is the same in both branches; the branch scaler changes how much the unclustered entries move relative to the null.}
\label{tab:s-adversarial-branch}
\centering
\scriptsize
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{@{}lrrrrr@{}}
\toprule
 & & \multicolumn{2}{c}{Classical} & \multicolumn{2}{c}{Quantum} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
Mechanism & Strength & $\mathcal I_X$ & $\mathcal I_{XF}$ & $\mathcal I_X$ & $\mathcal I_{XF}$ \\
\midrule
Mean shift & 0.02 & 0.00 & 0.00 & 0.01 & 0.10 \\
Mean shift & 0.05 & 0.04 & 0.04 & 0.10 & 0.37 \\
Mean shift & 0.10 & 0.30 & 0.34 & 0.37 & 0.58 \\
Mean shift & 0.25 & 0.72 & 0.72 & 0.84 & 0.85 \\
Mean shift & 0.50 & 0.85 & 0.86 & 0.91 & 0.93 \\
Scaling drift & 0.02 & 0.00 & 0.00 & 0.08 & 0.38 \\
Scaling drift & 0.05 & 0.14 & 0.14 & 0.49 & 0.69 \\
Scaling drift & 0.10 & 0.33 & 0.39 & 0.72 & 0.84 \\
Scaling drift & 0.25 & 0.47 & 0.57 & 0.94 & 0.94 \\
Scaling drift & 0.50 & 0.72 & 0.75 & 0.97 & 0.97 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_adversarial_detection.tex <==
\begin{table*}[!tbp]
\caption{Gate A: detection rate of the executed drift mechanisms (matched controls) and of their adaptive cluster-preserving variants (F5), 600 observations per row pooled over the eight environments, as union / 1.2.0 rule / conformal rule in the batch-level regimes, and exact item-aligned detection (prediction disagreement or confusion-profile delta) under $\mathcal I_{XFY}^{\star}$.}
\label{tab:s-adversarial-detection}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrllll@{}}
\toprule
Mechanism & Strength & $\mathcal I_X$ & $\mathcal I_{XF}$ & $\mathcal I_{XFY}$ & $\mathcal I_{XFY}^{\star}$ exact \\
\midrule
Mean shift (executed) & 0.02 & 1.00 / 1.00 / 1.00 & 1.00 / 1.00 / 0.97 & 1.00 / 0.99 / 0.97 & 0.36 \\
Mean shift (executed) & 0.05 & 1.00 / 1.00 / 1.00 & 1.00 / 1.00 / 1.00 & 1.00 / 1.00 / 1.00 & 0.50 \\
Mean shift (executed) & 0.10 & 1.00 / 1.00 / 1.00 & 1.00 / 1.00 / 1.00 & 1.00 / 1.00 / 1.00 & 0.62 \\
Mean shift (F5) & 0.02 & 0.01 / 0.01 / 0.01 & 0.10 / 0.06 / 0.06 & 0.10 / 0.06 / 0.06 & 0.32 \\
Mean shift (F5) & 0.05 & 0.10 / 0.08 / 0.08 & 0.31 / 0.26 / 0.24 & 0.31 / 0.24 / 0.22 & 0.45 \\
Mean shift (F5) & 0.10 & 0.40 / 0.34 / 0.34 & 0.60 / 0.52 / 0.48 & 0.60 / 0.50 / 0.45 & 0.60 \\
Mean shift (F5) & 0.25 & 0.82 / 0.79 / 0.79 & 0.87 / 0.82 / 0.80 & 0.87 / 0.81 / 0.79 & 0.74 \\
Mean shift (F5) & 0.50 & 0.91 / 0.89 / 0.89 & 0.94 / 0.91 / 0.90 & 0.94 / 0.91 / 0.89 & 0.79 \\
\addlinespace[1pt]
Scaling drift (executed) & 0.02 & 1.00 / 0.99 / 0.99 & 1.00 / 0.99 / 0.96 & 1.00 / 0.98 / 0.95 & 0.54 \\
Scaling drift (executed) & 0.05 & 1.00 / 1.00 / 1.00 & 1.00 / 1.00 / 0.99 & 1.00 / 1.00 / 0.99 & 0.61 \\
Scaling drift (executed) & 0.10 & 1.00 / 1.00 / 1.00 & 1.00 / 1.00 / 1.00 & 1.00 / 1.00 / 1.00 & 0.67 \\
Scaling drift (F5) & 0.02 & 0.07 / 0.05 / 0.05 & 0.28 / 0.24 / 0.23 & 0.28 / 0.23 / 0.22 & 0.47 \\
Scaling drift (F5) & 0.05 & 0.39 / 0.35 / 0.35 & 0.57 / 0.50 / 0.47 & 0.57 / 0.47 / 0.45 & 0.57 \\
Scaling drift (F5) & 0.10 & 0.61 / 0.56 / 0.56 & 0.71 / 0.67 / 0.66 & 0.71 / 0.66 / 0.65 & 0.64 \\
Scaling drift (F5) & 0.25 & 0.79 / 0.76 / 0.76 & 0.85 / 0.81 / 0.79 & 0.85 / 0.80 / 0.77 & 0.77 \\
Scaling drift (F5) & 0.50 & 0.91 / 0.88 / 0.88 & 0.95 / 0.90 / 0.88 & 0.95 / 0.89 / 0.86 & 0.87 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_adversarial_env.tex <==
\begin{table*}[!tbp]
\caption{Gate A: per-environment detection rate of the adaptive variants under the conformal rule in $\mathcal I_{XF}$ (rows pooled over models, dimensions, splits and seeds), and mean fraction of entries the attacker perturbs in that environment.}
\label{tab:s-adversarial-env}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrrrrrrrrrrr@{}}
\toprule
 & & \multicolumn{5}{c}{Mean shift} & \multicolumn{5}{c}{Scaling drift} \\
\cmidrule(lr){3-7}\cmidrule(lr){8-12}
Environment & Perturbed & 0.02 & 0.05 & 0.10 & 0.25 & 0.50 & 0.02 & 0.05 & 0.10 & 0.25 & 0.50 \\
\midrule
E1 CICIDS ID 256 & 0.40 & 0.03 & 0.43 & 0.90 & 1.00 & 1.00 & 0.50 & 0.67 & 1.00 & 1.00 & 1.00 \\
E2 UNSW-NB15 ID & 0.45 & 0.13 & 0.33 & 0.48 & 0.93 & 0.99 & 0.24 & 0.50 & 0.77 & 0.88 & 0.99 \\
E3 ToN-IoT ID & 0.23 & 0.03 & 0.24 & 0.47 & 0.77 & 0.92 & 0.20 & 0.42 & 0.57 & 0.75 & 0.88 \\
E4 CICIDS Tue$\to$Wed & 0.40 & 0.00 & 0.00 & 0.00 & 0.25 & 0.55 & 0.00 & 0.82 & 1.00 & 1.00 & 1.00 \\
E5 CICIDS Tue$\to$Fri-PortScan & 0.19 & 0.00 & 0.02 & 0.32 & 0.65 & 0.75 & 0.00 & 0.12 & 0.25 & 0.43 & 0.60 \\
E6 CICIDS Wed$\to$Thu-Web & 0.30 & 0.05 & 0.27 & 0.75 & 0.98 & 1.00 & 0.37 & 0.53 & 0.82 & 1.00 & 1.00 \\
E7 CICIDS Wed$\to$Fri-AM & 0.16 & 0.00 & 0.08 & 0.37 & 0.95 & 0.88 & 0.08 & 0.18 & 0.30 & 0.50 & 0.60 \\
E8 UNSW temporal OOD & 0.45 & 0.18 & 0.43 & 0.60 & 0.78 & 1.00 & 0.42 & 0.50 & 0.57 & 0.70 & 0.90 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_adversarial_materiality.tex <==
\begin{table*}[!tbp]
\caption{Gate A: prediction-change rate (item-aligned disagreement $>0$), material fraction at $|\Delta_R|>0$, $\ge0.02$ and $\ge0.05$, mean $|\Delta_R|$, fraction of rows whose balanced accuracy rose, and mean fraction of feature entries the attacker perturbs (the executed mechanisms perturb every entry).}
\label{tab:s-adversarial-materiality}
\centering
\scriptsize
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
Mechanism & Strength & Pred.\ change & Mat.\ $0^{+}$ & Mat.\ 0.02 & Mat.\ 0.05 & Mean $|\Delta_R|$ & Raised & Perturbed \\
\midrule
Mean shift (executed) & 0.02 & 0.36 & 0.33 & 0.10 & 0.06 & 0.011 & 0.13 & -- \\
Mean shift (executed) & 0.05 & 0.50 & 0.46 & 0.20 & 0.11 & 0.026 & 0.20 & -- \\
Mean shift (executed) & 0.10 & 0.62 & 0.59 & 0.35 & 0.24 & 0.054 & 0.20 & -- \\
Mean shift (F5) & 0.02 & 0.32 & 0.29 & 0.03 & 0.00 & 0.003 & 0.14 & 0.33 \\
Mean shift (F5) & 0.05 & 0.45 & 0.40 & 0.10 & 0.01 & 0.006 & 0.20 & 0.33 \\
Mean shift (F5) & 0.10 & 0.60 & 0.54 & 0.22 & 0.05 & 0.014 & 0.22 & 0.33 \\
Mean shift (F5) & 0.25 & 0.74 & 0.69 & 0.42 & 0.22 & 0.033 & 0.25 & 0.33 \\
Mean shift (F5) & 0.50 & 0.79 & 0.76 & 0.52 & 0.35 & 0.053 & 0.18 & 0.33 \\
\addlinespace[1pt]
Scaling drift (executed) & 0.02 & 0.54 & 0.48 & 0.23 & 0.14 & 0.032 & 0.17 & -- \\
Scaling drift (executed) & 0.05 & 0.61 & 0.57 & 0.42 & 0.30 & 0.063 & 0.17 & -- \\
Scaling drift (executed) & 0.10 & 0.67 & 0.64 & 0.50 & 0.41 & 0.096 & 0.19 & -- \\
Scaling drift (F5) & 0.02 & 0.47 & 0.40 & 0.11 & 0.02 & 0.008 & 0.15 & 0.33 \\
Scaling drift (F5) & 0.05 & 0.57 & 0.52 & 0.27 & 0.11 & 0.019 & 0.16 & 0.33 \\
Scaling drift (F5) & 0.10 & 0.64 & 0.58 & 0.36 & 0.21 & 0.030 & 0.18 & 0.33 \\
Scaling drift (F5) & 0.25 & 0.77 & 0.72 & 0.47 & 0.33 & 0.048 & 0.19 & 0.33 \\
Scaling drift (F5) & 0.50 & 0.87 & 0.81 & 0.53 & 0.35 & 0.060 & 0.18 & 0.33 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_adversarial_policy.tex <==
\begin{table*}[!tbp]
\caption{Gate A: materially altered audit results served under P1 union, P2 conformal and P3 sensor-coverage-complete relative to declared evidence dimensions per regime, summed over mechanisms and strengths (structural-sensitivity endpoint $|\Delta_R|>0$). Under $\mathcal I_{XFY}^{\star}$ every material row carries a prediction change and is blocked.}
\label{tab:s-adversarial-policy}
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lrrrr@{}}
\toprule
Regime & Material & P1 union & P2 conformal & P3 abst. \\
\midrule
\multicolumn{5}{@{}l}{\emph{Executed mechanisms (1,800 rows)}} \\
$\mathcal I_X$ & 1,848 & 0 & 0 & 0 \\
$\mathcal I_{XF}$ & 1,848 & 0 & 6 & 0 \\
$\mathcal I_{XFY}$ & 1,848 & 0 & 10 & 10 \\
$\mathcal I_{XFY}^{\star}$ & 1,848 & 0 & 0 & 0 \\
\addlinespace[1pt]
\multicolumn{5}{@{}l}{\emph{Cluster-preserving F5 (6,000 rows)}} \\
$\mathcal I_X$ & 3,418 & 1,207 & 1,328 & 0 \\
$\mathcal I_{XF}$ & 3,418 & 719 & 959 & 0 \\
$\mathcal I_{XFY}$ & 3,418 & 716 & 1,006 & 1,006 \\
$\mathcal I_{XFY}^{\star}$ & 3,418 & 0 & 0 & 0 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_clean.tex <==
\begin{table*}[!t]
\caption{Gates P and T: clean balanced accuracy (SVC / ZZ, mean over five split clusters) per configuration and dimension, and the distribution of cross-validated regularisation constants over the 30 cells of each tuned environment (SVC also selects $\gamma$; see the artifact table).}
\label{tab:s-clean}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}llll@{}}
\toprule
Condition & $d=8$ & $d=10$ & $d=12$ \\
\midrule
P0 reference (standard / minmax2$\pi$) & 0.753 / 0.734 & 0.747 / 0.728 & 0.778 / 0.747 \\
PA standard / standard & 0.753 / 0.727 & 0.747 / 0.720 & 0.778 / 0.727 \\
PB minmax2$\pi$ / minmax2$\pi$ & 0.751 / 0.734 & 0.750 / 0.728 & 0.756 / 0.747 \\
CICIDS ID, both tuned (CV5) & 0.741 / 0.750 & 0.746 / 0.781 & 0.780 / 0.802 \\
UNSW OOD, frozen defaults & 0.748 / 0.760 & 0.754 / 0.766 & 0.755 / 0.769 \\
UNSW OOD, both tuned (CV5) & 0.739 / 0.759 & 0.723 / 0.757 & 0.736 / 0.770 \\
\midrule
Tuned environment & \multicolumn{2}{l}{QSVC $C$ selections} & SVC $C$ selections \\
\midrule
CICIDS ID & \multicolumn{2}{l}{$C=0.1$: 3, $C=1$: 4, $C=10$: 6, $C=100$: 17} & $C=0.1$: 1, $C=1$: 6, $C=10$: 15, $C=100$: 8 \\
UNSW OOD & \multicolumn{2}{l}{$C=1$: 17, $C=10$: 13} & $C=0.1$: 1, $C=1$: 2, $C=10$: 15, $C=100$: 12 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_clean_by_environment.tex <==
% Presentation-only summary derived from frozen expansion_unique_observations.csv.
\begin{table}[!t]
\caption{Clean balanced accuracy by expansion environment. Values are mean
[range] over five split clusters after averaging the prespecified
dimension/model/model-seed cells within each cluster.}
\label{tab:s-clean-env}
\centering
\footnotesize
\begin{tabular}{@{}lc@{}}
\toprule
Environment & Clean BA mean [range] \\
\midrule
E1 CICIDS scale/ID & 0.762 [0.756, 0.766] \\
E2 UNSW-NB15 ID & 0.766 [0.738, 0.800] \\
E3 ToN-IoT ID & 0.752 [0.716, 0.807] \\
E4 CICIDS Tue$\rightarrow$Wed & 0.492 [0.480, 0.520] \\
E5 CICIDS Tue$\rightarrow$Fri-PortScan & 0.590 [0.565, 0.615] \\
E6 CICIDS Wed$\rightarrow$Thu-Web & 0.483 [0.454, 0.518] \\
E7 CICIDS Wed$\rightarrow$Fri-AM & 0.459 [0.431, 0.493] \\
E8 UNSW temporal OOD & 0.759 [0.743, 0.775] \\
\bottomrule
\end{tabular}
\end{table}


==> tables/s_composition.tex <==
\begin{table}[!tbp]
\caption{Composition of the frozen four-contract envelopes with the policy layer under $\mathcal I_{XFY}^{\star}$ (lattice maximum). Approved rewrites and approved stochastic estimation are not exact violations; the contract's own \texttt{hold} for the approved emulator is preserved.}
\label{tab:s-composition}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lllll@{}}
\toprule
Scenario & Contract & Exact viol. & Policy & Composed \\
\midrule
Clean & \texttt{allow} & no & \texttt{allow} & \texttt{allow} \\
Approved transpilation & \texttt{allow} & no & \texttt{allow} & \texttt{allow} \\
Parameterized circuit mutation & \texttt{block} & yes & \texttt{block} & \texttt{block} \\
PSD-preserving kernel substitution & \texttt{block} & yes & \texttt{block} & \texttt{block} \\
Prior-preserving label corruption & \texttt{block} & yes & \texttt{block} & \texttt{block} \\
Approved 256-shot emulator & \texttt{hold} & no & \texttt{allow} & \texttt{hold} \\
\bottomrule
\end{tabular}
\end{table}


==> tables/s_detection.tex <==
\begin{table*}[!t]
\caption{Gate N: detection rate of each regime on the frozen \texttt{paper\_core} observations (all environments, dimensions and models pooled; 600 observations per intervention row) at the null-calibrated thresholds, and firing rate on the in-place near-null controls. Batch-level regimes use calibrated distributional sensors; item-aligned regimes use exact zero thresholds on item-wise deltas.}
\label{tab:s-detection}
\centering
\footnotesize
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
Intervention & $\mathcal I_X$ & $\mathcal I_{XF}$ & $\mathcal I_{Y_m}$ & $\mathcal I_{XFY}$ & $\mathcal I_{XF}$ item & $\mathcal I_{XFY}$ item \\
\midrule
Feature sign flip 0.02 & 0.118 & 0.192 & 0.000 & 0.200 & 0.793 & 0.793 \\
Feature sign flip 0.05 & 0.532 & 0.640 & 0.000 & 0.643 & 0.867 & 0.867 \\
Feature sign flip 0.10 & 0.757 & 0.877 & 0.000 & 0.878 & 0.907 & 0.907 \\
Mean shift 0.02 & 1.000 & 1.000 & 0.000 & 1.000 & 0.357 & 0.357 \\
Mean shift 0.05 & 1.000 & 1.000 & 0.000 & 1.000 & 0.500 & 0.500 \\
Mean shift 0.10 & 1.000 & 1.000 & 0.000 & 1.000 & 0.618 & 0.618 \\
Scaling drift 0.02 & 1.000 & 1.000 & 0.000 & 1.000 & 0.537 & 0.537 \\
Scaling drift 0.05 & 1.000 & 1.000 & 0.000 & 1.000 & 0.608 & 0.608 \\
Scaling drift 0.10 & 1.000 & 1.000 & 0.000 & 1.000 & 0.668 & 0.668 \\
Feature dropout 0.02 & 0.000 & 0.000 & 0.000 & 0.000 & 0.488 & 0.488 \\
Feature dropout 0.05 & 0.000 & 0.022 & 0.000 & 0.022 & 0.705 & 0.705 \\
Feature dropout 0.10 & 0.000 & 0.062 & 0.000 & 0.062 & 0.763 & 0.763 \\
Prior-preserving label flip 0.02 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 1.000 \\
Prior-preserving label flip 0.05 & 0.000 & 0.000 & 0.000 & 0.002 & 0.000 & 1.000 \\
Prior-preserving label flip 0.10 & 0.000 & 0.000 & 0.000 & 0.033 & 0.000 & 1.000 \\
Random label flip 0.02 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 1.000 \\
Random label flip 0.05 & 0.000 & 0.000 & 0.000 & 0.003 & 0.000 & 1.000 \\
Random label flip 0.10 & 0.000 & 0.000 & 0.000 & 0.033 & 0.000 & 1.000 \\
\midrule
Near-null Gaussian $\sigma=0.001$ & 0.713 & 0.713 & 0.000 & 0.713 & 0.042 & 0.042 \\
Near-null scaling $\alpha=0.001$ & 0.879 & 0.882 & 0.000 & 0.882 & 0.099 & 0.099 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_family_decomposition.tex <==
\begin{table}[!tbp]
\caption{Gate F: decomposition of the pooled excess of the 1.2.0 rule over the nominal 0.05 into rule bias (1.2.0 rate minus conformal rate on the same draws) and design effect (conformal rate minus nominal), and both rules under 30 exchangeable random re-splits of the 400 pooled draws of every cell (seed 20260907), where the roles are assigned by a uniform random permutation and any excess of the 1.2.0 rule is its own bias; the conformal rule must stay at or below $10/201=0.0498$.}
\label{tab:s-family-decomposition}
\centering
\scriptsize
\setlength{\tabcolsep}{2.6pt}
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
Regime & 1.2.0 & Conformal & Rule bias & Design & Re-split 1.2.0 & Re-split conf. \\
\midrule
$\mathcal I_X$ & 0.061 & 0.056 & +0.005 & +0.006 & 0.052 & 0.044 \\
$\mathcal I_{XF}$ & 0.073 & 0.058 & +0.015 & +0.008 & 0.058 & 0.042 \\
$\mathcal I_{Y_m}$ & 0.048 & 0.048 & +0.000 & -0.003 & 0.040 & 0.040 \\
$\mathcal I_{XFY}$ & 0.079 & 0.053 & +0.025 & +0.003 & 0.059 & 0.036 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/s_family_detection.tex <==
\begin{table*}[!tbp]
\caption{Gate F: detection rate on the frozen \texttt{paper\_core} observations (600 per intervention row, eight environments pooled) and firing rate on the near-null in-place controls, as union rule / 1.2.0 rule / conformal rule. Within this executed design, the conformal rule trades a small loss of detection for the descriptive decision-level false-action rates of Table~\ref{tab:s-family-fpr}.}
\label{tab:s-family-detection}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lllll@{}}
\toprule
Intervention & $\mathcal I_X$ & $\mathcal I_{XF}$ & $\mathcal I_{Y_m}$ & $\mathcal I_{XFY}$ \\
\midrule
Feature sign flip 0.02 & 0.12 / 0.09 / 0.09 & 0.19 / 0.15 / 0.13 & 0.00 / 0.00 / 0.00 & 0.20 / 0.15 / 0.12 \\
Feature sign flip 0.05 & 0.53 / 0.47 / 0.47 & 0.64 / 0.56 / 0.52 & 0.00 / 0.00 / 0.00 & 0.64 / 0.53 / 0.47 \\
Feature sign flip 0.10 & 0.76 / 0.72 / 0.72 & 0.88 / 0.85 / 0.84 & 0.00 / 0.00 / 0.00 & 0.88 / 0.84 / 0.83 \\
Mean shift 0.02 & 1.00 / 1.00 / 1.00 & 1.00 / 1.00 / 0.97 & 0.00 / 0.00 / 0.00 & 1.00 / 0.99 / 0.97 \\
Mean shift 0.05 & 1.00 / 1.00 / 1.00 & 1.00 / 1.00 / 1.00 & 0.00 / 0.00 / 0.00 & 1.00 / 1.00 / 1.00 \\
Mean shift 0.10 & 1.00 / 1.00 / 1.00 & 1.00 / 1.00 / 1.00 & 0.00 / 0.00 / 0.00 & 1.00 / 1.00 / 1.00 \\
Scaling drift 0.02 & 1.00 / 0.99 / 0.99 & 1.00 / 0.99 / 0.96 & 0.00 / 0.00 / 0.00 & 1.00 / 0.98 / 0.95 \\
Scaling drift 0.05 & 1.00 / 1.00 / 1.00 & 1.00 / 1.00 / 0.99 & 0.00 / 0.00 / 0.00 & 1.00 / 1.00 / 0.99 \\
Scaling drift 0.10 & 1.00 / 1.00 / 1.00 & 1.00 / 1.00 / 1.00 & 0.00 / 0.00 / 0.00 & 1.00 / 1.00 / 1.00 \\
Feature dropout 0.02 & 0.00 / 0.00 / 0.00 & 0.00 / 0.00 / 0.00 & 0.00 / 0.00 / 0.00 & 0.00 / 0.00 / 0.00 \\
Feature dropout 0.05 & 0.00 / 0.00 / 0.00 & 0.02 / 0.01 / 0.01 & 0.00 / 0.00 / 0.00 & 0.02 / 0.01 / 0.01 \\
Feature dropout 0.10 & 0.00 / 0.00 / 0.00 & 0.06 / 0.04 / 0.03 & 0.00 / 0.00 / 0.00 & 0.06 / 0.03 / 0.03 \\
Prior-preserving label flip 0.02 & 0.00 / 0.00 / 0.00 & 0.00 / 0.00 / 0.00 & 0.00 / 0.00 / 0.00 & 0.00 / 0.00 / 0.00 \\
Prior-preserving label flip 0.05 & 0.00 / 0.00 / 0.00 & 0.00 / 0.00 / 0.00 & 0.00 / 0.00 / 0.00 & 0.00 / 0.00 / 0.00 \\
Prior-preserving label flip 0.10 & 0.00 / 0.00 / 0.00 & 0.00 / 0.00 / 0.00 & 0.00 / 0.00 / 0.00 & 0.03 / 0.01 / 0.01 \\
Random label flip 0.02 & 0.00 / 0.00 / 0.00 & 0.00 / 0.00 / 0.00 & 0.00 / 0.00 / 0.00 & 0.00 / 0.00 / 0.00 \\
Random label flip 0.05 & 0.00 / 0.00 / 0.00 & 0.00 / 0.00 / 0.00 & 0.00 / 0.00 / 0.00 & 0.00 / 0.00 / 0.00 \\
Random label flip 0.10 & 0.00 / 0.00 / 0.00 & 0.00 / 0.00 / 0.00 & 0.00 / 0.00 / 0.00 & 0.03 / 0.01 / 0.01 \\
\midrule
Near-null Gaussian $\sigma=0.001$ & 0.65 / 0.49 / 0.45 & 0.65 / 0.44 / 0.41 & 0.00 / 0.00 / 0.00 & 0.65 / 0.43 / 0.41 \\
Near-null scaling $\alpha=0.001$ & 0.86 / 0.68 / 0.64 & 0.86 / 0.64 / 0.62 & 0.00 / 0.00 / 0.00 & 0.86 / 0.62 / 0.58 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_family_fpr.tex <==
\begin{table}[!tbp]
\caption{Gate F: decision-level false-action rate on clean draws from evaluation pools disjoint from the calibration pools (12,000 in the primary aggregate; nominal $\alpha=0.05$ per decision; exact level of the conformal rule $10/201=0.0498$ under exchangeability) for the union of per-sensor rules, the superseded asymmetric family rule and the adopted conformal family rule. Pooled rates are descriptive because resampled draws within a pool may overlap; the last column is the range of the per-environment cluster means of the conformal rule (five split clusters each). E1 is never excluded from the primary aggregate.}
\label{tab:s-family-fpr}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrrrl@{}}
\toprule
Regime & Union & 1.2.0 rule & Conformal & Env.\ cluster means (conformal) \\
\midrule
\multicolumn{5}{@{}l}{\emph{All eight environments (primary)}} \\
$\mathcal I_X$ & 0.125 & 0.061 & 0.056 & 0.023--0.125 \\
$\mathcal I_{XF}$ & 0.203 & 0.073 & 0.058 & 0.023--0.115 \\
$\mathcal I_{Y_m}$ & 0.048 & 0.048 & 0.048 & 0.025--0.070 \\
$\mathcal I_{XFY}$ & 0.259 & 0.079 & 0.053 & 0.034--0.123 \\
\addlinespace[1pt]
\multicolumn{5}{@{}l}{\emph{Seven environments, E1 excluded (sensitivity)}} \\
$\mathcal I_X$ & 0.116 & 0.053 & 0.048 & 0.023--0.092 \\
$\mathcal I_{XF}$ & 0.199 & 0.067 & 0.052 & 0.023--0.081 \\
$\mathcal I_{Y_m}$ & 0.048 & 0.048 & 0.048 & 0.025--0.070 \\
$\mathcal I_{XFY}$ & 0.251 & 0.071 & 0.045 & 0.034--0.065 \\
\addlinespace[1pt]
\multicolumn{5}{@{}l}{\emph{E1 only (256-row draws from 322-row halves)}} \\
$\mathcal I_X$ & 0.203 & 0.133 & 0.125 & 0.125--0.125 \\
$\mathcal I_{XF}$ & 0.245 & 0.125 & 0.115 & 0.115--0.115 \\
$\mathcal I_{Y_m}$ & 0.045 & 0.045 & 0.045 & 0.045--0.045 \\
$\mathcal I_{XFY}$ & 0.331 & 0.146 & 0.123 & 0.123--0.123 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\end{table}


==> tables/s_family_fpr_env.tex <==
\begin{table*}[!tbp]
\caption{Gate F: per-environment false-alarm rate of the conformal family rule (cluster mean over the five split clusters with the two-sided 95\% $t$ interval, four degrees of freedom). $n$ is the batch size; ``disjoint'' is the number of mutually disjoint batches that one pool half can supply, an upper bound on the effective number of independent draws among the 20 per run (E1: one). The union and 1.2.0 cluster means are in Table~\ref{tab:s-family-fpr-env-rules}.}
\label{tab:s-family-fpr-env}
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}lrrllll@{}}
\toprule
Environment & $n$ & disj. & $\mathcal I_X$ & $\mathcal I_{XF}$ & $\mathcal I_{Y_m}$ & $\mathcal I_{XFY}$ \\
\midrule
E1 CICIDS ID 256 & 256 & 1 & 0.125 [-0.05,0.30] & 0.115 [-0.03,0.26] & 0.045 [-0.05,0.14] & 0.123 [0.00,0.24] \\
E2 UNSW-NB15 ID & 128 & 3 & 0.023 [-0.02,0.06] & 0.042 [0.01,0.07] & 0.070 [0.01,0.13] & 0.035 [0.01,0.06] \\
E3 ToN-IoT ID & 128 & 3 & 0.065 [-0.02,0.15] & 0.075 [0.01,0.15] & 0.070 [0.01,0.13] & 0.062 [0.01,0.12] \\
E4 CICIDS Tue$\to$Wed & 128 & 11 & 0.092 [-0.01,0.19] & 0.081 [0.01,0.15] & 0.025 [-0.01,0.06] & 0.065 [0.02,0.11] \\
E5 CICIDS Tue$\to$Fri-PortScan & 128 & 11 & 0.032 [-0.01,0.08] & 0.023 [-0.02,0.06] & 0.025 [-0.01,0.06] & 0.037 [-0.00,0.08] \\
E6 CICIDS Wed$\to$Thu-Web & 128 & 11 & 0.044 [0.00,0.09] & 0.036 [-0.01,0.08] & 0.025 [-0.01,0.06] & 0.037 [0.00,0.07] \\
E7 CICIDS Wed$\to$Fri-AM & 128 & 11 & 0.049 [0.01,0.09] & 0.041 [0.02,0.06] & 0.025 [-0.01,0.06] & 0.034 [0.02,0.05] \\
E8 UNSW temporal OOD & 128 & 11 & 0.043 [-0.03,0.12] & 0.049 [0.02,0.08] & 0.050 [-0.01,0.11] & 0.041 [0.03,0.05] \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_family_fpr_env_rules.tex <==
\begin{table}[!tbp]
\caption{Gate F: per-environment cluster means of the union rule / the superseded 1.2.0 rule, for comparison with Table~\ref{tab:s-family-fpr-env} (environment codes as there).}
\label{tab:s-family-fpr-env-rules}
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{@{}lllll@{}}
\toprule
Env. & $\mathcal I_X$ & $\mathcal I_{XF}$ & $\mathcal I_{Y_m}$ & $\mathcal I_{XFY}$ \\
\midrule
E1 & 0.203 / 0.133 & 0.245 / 0.125 & 0.045 / 0.045 & 0.331 / 0.146 \\
E2 & 0.063 / 0.025 & 0.135 / 0.051 & 0.070 / 0.070 & 0.210 / 0.054 \\
E3 & 0.215 / 0.071 & 0.280 / 0.088 & 0.070 / 0.070 & 0.358 / 0.102 \\
E4 & 0.150 / 0.098 & 0.230 / 0.095 & 0.025 / 0.025 & 0.254 / 0.102 \\
E5 & 0.066 / 0.039 & 0.160 / 0.045 & 0.025 / 0.025 & 0.197 / 0.046 \\
E6 & 0.070 / 0.044 & 0.163 / 0.054 & 0.025 / 0.025 & 0.181 / 0.054 \\
E7 & 0.133 / 0.060 & 0.212 / 0.063 & 0.025 / 0.025 & 0.257 / 0.061 \\
E8 & 0.072 / 0.043 & 0.192 / 0.065 & 0.050 / 0.050 & 0.237 / 0.065 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/s_family_split.tex <==
\begin{table}[!tbp]
\caption{Sensitivity S1: split construction (reference draws 01--10 of each run define the rank transform, calibration draws 11--20 give the null family scores; p-value resolution $1/101$) on the same 12,000 evaluation draws. Valid under the same premise but using half of the draws for each role; the adopted rule is the full conformal one.}
\label{tab:s-family-split}
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lrrr@{}}
\toprule
Regime & Draws & Fires & Pooled rate \\
\midrule
$\mathcal I_X$ & 12,000 & 592 & 0.049 \\
$\mathcal I_{XF}$ & 12,000 & 470 & 0.039 \\
$\mathcal I_{Y_m}$ & 12,000 & 804 & 0.067 \\
$\mathcal I_{XFY}$ & 12,000 & 403 & 0.034 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/s_fpr.tex <==
\begin{table}[!t]
\caption{Gate N: empirical false-action rate of the null-calibrated sensors and batch-level regimes on 12,000 clean draws from evaluation pools disjoint from the calibration pools (all eight environments pooled; nominal $\alpha=0.05$ per sensor). Resampled draws within a pool may overlap. Intervals are descriptive Clopper--Pearson 95\% intervals: draws within a cell share a pool half and are not independent. Regime rows are unions without correction.}
\label{tab:s-fpr}
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lrrl@{}}
\toprule
Sensor / regime & Fires & Rate & 95\% CI \\
\midrule
Feature JSD & 600 & 0.050 & [0.046, 0.054] \\
Feature MMD & 822 & 0.069 & [0.064, 0.073] \\
KS rejection rate & 342 & 0.029 & [0.026, 0.032] \\
Score JSD & 668 & 0.056 & [0.052, 0.060] \\
Prediction-rate shift & 520 & 0.043 & [0.040, 0.047] \\
Prediction JSD & 586 & 0.049 & [0.045, 0.053] \\
Label prior shift & 570 & 0.048 & [0.044, 0.051] \\
Label JSD & 570 & 0.048 & [0.044, 0.051] \\
Confusion profile $L_1$ & 517 & 0.043 & [0.040, 0.047] \\
Confusion profile JSD & 638 & 0.053 & [0.049, 0.057] \\
\midrule
$\mathcal I_X$ (any sensor) & 1500 & 0.125 & [0.119, 0.131] \\
$\mathcal I_{XF}$ (any sensor) & 2438 & 0.203 & [0.196, 0.210] \\
$\mathcal I_{Y_m}$ (any sensor) & 570 & 0.048 & [0.044, 0.051] \\
$\mathcal I_{XFY}$ (any sensor) & 3113 & 0.259 & [0.252, 0.267] \\
\bottomrule
\end{tabular}
\end{table}


==> tables/s_fpr_env.tex <==
\begin{table*}[!t]
\caption{Gate N: per-environment false-alarm rates on 1,200 evaluation draws (three dimensions, two or four models, 200 draws per cell). Sensor range is the minimum and maximum per-sensor rate in the environment; regime columns are batch-level unions. E1 draws 256 rows from 322-row pool halves and is indicative only.}
\label{tab:s-fpr-env}
\centering
\footnotesize
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}lrrlrrrr@{}}
\toprule
Environment & $n$ & Pool half & Sensor range & $\mathcal I_X$ & $\mathcal I_{XF}$ & $\mathcal I_{Y_m}$ & $\mathcal I_{XFY}$ \\
\midrule
E1 CICIDS ID 256 & 256 & 322 & 0.023--0.130 & 0.203 & 0.245 & 0.045 & 0.331 \\
E2 UNSW-NB15 ID & 128 & 386 & 0.008--0.070 & 0.063 & 0.135 & 0.070 & 0.210 \\
E3 ToN-IoT ID & 128 & 386 & 0.025--0.172 & 0.215 & 0.280 & 0.070 & 0.358 \\
E4 Tue$\to$Wed & 128 & 1436 & 0.025--0.082 & 0.150 & 0.230 & 0.025 & 0.254 \\
E5 Tue$\to$Fri-PortScan & 128 & 1436 & 0.018--0.051 & 0.066 & 0.160 & 0.025 & 0.198 \\
E6 Wed$\to$Thu-Web & 128 & 1436 & 0.013--0.057 & 0.070 & 0.163 & 0.025 & 0.181 \\
E7 Wed$\to$Fri-AM & 128 & 1436 & 0.025--0.066 & 0.133 & 0.212 & 0.025 & 0.258 \\
E8 UNSW temporal OOD & 128 & 1436 & 0.032--0.092 & 0.072 & 0.192 & 0.050 & 0.237 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_geometry_sensitivity.tex <==
% Generated by build_v135_geometry_sensitivity.py; do not edit.
\begin{table*}[!tbp]
\caption{Geometry-aligned sensitivity under the adopted full-conformal family rule (600 observations per intervention). Material is $|\Delta_R|>0$ and is common to both regimes.}
\label{tab:s-geometry-feature}
\centering\footnotesize
\begin{tabular}{llrrr}
\toprule
Intervention & Strength & $\mathcal I_X$ response & $\mathcal I_{XF}$ response & Material fraction \\
\midrule
Tiny Gaussian & 0.001 & 0.637 & 0.568 & 0.045 \\
Tiny scaling & 0.001 & 0.822 & 0.808 & 0.095 \\
Mean shift & 0.02 & 1.000 & 0.993 & 0.363 \\
Mean shift & 0.05 & 1.000 & 1.000 & 0.508 \\
Mean shift & 0.10 & 1.000 & 1.000 & 0.622 \\
Scaling drift & 0.02 & 1.000 & 0.997 & 0.512 \\
Scaling drift & 0.05 & 1.000 & 1.000 & 0.612 \\
Scaling drift & 0.10 & 1.000 & 1.000 & 0.680 \\
Feature dropout & 0.02 & 0.057 & 0.068 & 0.442 \\
Feature dropout & 0.05 & 0.085 & 0.137 & 0.680 \\
Feature dropout & 0.10 & 0.212 & 0.320 & 0.768 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[!tbp]
\caption{Matched geometry-aligned Gate A sensitivity. Lower cells count environment/split cells in which adaptive response is below its matched control; there are 40 cells per regime. Material nonresponse is conditional on an adaptive material row.}
\label{tab:s-geometry-gatea}
\centering\scriptsize
\begin{tabular}{llrrrrrr}
\toprule
Mechanism & Strength & $\mathcal I_X$ ctrl./adapt. & $\mathcal I_{XF}$ ctrl./adapt. & Lower $\mathcal I_X$ & Lower $\mathcal I_{XF}$ & Adaptive material & Material nonresponse range \\
\midrule
Mean shift & 0.02 & 1.000/0.185 & 0.993/0.298 & 40/40 & 39/40 & 0.262 & 0.637--0.834 \\
Mean shift & 0.05 & 1.000/0.392 & 1.000/0.535 & 37/40 & 38/40 & 0.448 & 0.353--0.576 \\
Mean shift & 0.10 & 1.000/0.620 & 1.000/0.723 & 29/40 & 31/40 & 0.593 & 0.216--0.340 \\
Scaling drift & 0.02 & 1.000/0.330 & 0.997/0.488 & 40/40 & 40/40 & 0.417 & 0.288--0.564 \\
Scaling drift & 0.05 & 1.000/0.587 & 1.000/0.693 & 29/40 & 30/40 & 0.558 & 0.167--0.328 \\
Scaling drift & 0.10 & 1.000/0.750 & 1.000/0.823 & 25/40 & 26/40 & 0.667 & 0.060--0.140 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_labelpath.tex <==
\begin{table}[!t]
\caption{Gate N: label-path interventions in the frozen expansion; number of observations on which each regime fires after calibration (batch-level) or by exact item-aligned comparison.}
\label{tab:s-labelpath}
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
Subset & $n$ & $\mathcal I_X$ & $\mathcal I_{XF}$ & $\mathcal I_{Y_m}$ & $\mathcal I_{XFY}$ & item-aligned \\
\midrule
All label interventions & 3,600 & 0 & 0 & 0 & 43 & 3,600 \\
Prior-preserving & 1,800 & 0 & 0 & 0 & 21 & 1,800 \\
Positive conclusion impact & 2,184 & 0 & 0 & 0 & 40 & 2,184 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/s_mass.tex <==
\begin{table}[!t]
\caption{Cluster structure of the frozen evaluation batches (mean over the 30 cells of each environment, standardized projected features): fraction of near-duplicate rows, and the largest fraction of rows within a window of 0.01 or 0.001 standard deviations in any feature (max) or on average over features (mean).}
\label{tab:s-mass}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrrrr@{}}
\toprule
Environment & Dup.\ rows & Max 0.01 & Mean 0.01 & Max 0.001 \\
\midrule
E1 CICIDS ID 256 & 0.074 & 0.825 & 0.562 & 0.648 \\
E2 UNSW-NB15 ID & 0.114 & 0.735 & 0.458 & 0.514 \\
E3 ToN-IoT ID & 0.257 & 0.870 & 0.466 & 0.571 \\
E4 Tue$\to$Wed & 0.054 & 0.766 & 0.489 & 0.480 \\
E5 Tue$\to$Fri-PortScan & 0.129 & 0.872 & 0.747 & 0.822 \\
E6 Wed$\to$Thu-Web & 0.004 & 0.827 & 0.433 & 0.696 \\
E7 Wed$\to$Fri-AM & 0.026 & 0.769 & 0.670 & 0.663 \\
E8 UNSW temporal OOD & 0.100 & 0.694 & 0.437 & 0.477 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/s_paired.tex <==
\begin{table*}[!t]
\caption{Gates P and T: within-split ZZ-minus-SVC difference in suite-average balanced-accuracy conclusion impact, mean with 95\% $t$ interval over five split clusters and number of positive clusters. CICIDS ID reference is the re-executed P0 configuration; UNSW OOD reference is the frozen 1.0.0 environment E8.}
\label{tab:s-paired}
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}llll@{}}
\toprule
Condition & $d=8$ & $d=10$ & $d=12$ \\
\midrule
P0 reference (standard / minmax2$\pi$) & 0.0245 [0.0069, 0.0422] (5/5) & 0.0348 [0.0176, 0.0520] (5/5) & 0.0407 [0.0305, 0.0509] (5/5) \\
PA standard / standard & 0.0070 [0.0014, 0.0125] (5/5) & 0.0130 [0.0041, 0.0219] (5/5) & 0.0111 [0.0052, 0.0170] (5/5) \\
PB minmax2$\pi$ / minmax2$\pi$ & 0.0238 [0.0054, 0.0423] (5/5) & 0.0323 [0.0156, 0.0491] (5/5) & 0.0396 [0.0261, 0.0531] (5/5) \\
CICIDS ID, both tuned (CV5) & 0.0426 [0.0094, 0.0757] (5/5) & 0.0713 [0.0494, 0.0932] (5/5) & 0.0776 [0.0610, 0.0943] (5/5) \\
UNSW OOD, frozen defaults & 0.0226 [0.0148, 0.0304] (5/5) & 0.0379 [0.0260, 0.0498] (5/5) & 0.0483 [0.0400, 0.0565] (5/5) \\
UNSW OOD, both tuned (CV5) & 0.0229 [0.0103, 0.0356] (5/5) & 0.0348 [0.0205, 0.0492] (5/5) & 0.0459 [0.0371, 0.0546] (5/5) \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_policy_family.tex <==
\begin{table*}[!tbp]
\caption{Gate D: materially altered audit results served / material observations by intervention mechanism under the conformal-rule policy P2, nominally calibrated under exchangeability (structural-sensitivity endpoint $|\Delta_R|>0$).}
\label{tab:s-policy-family}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrrrr@{}}
\toprule
Regime & Evaluation-label & Sign flip & Mean shift / scaling & Feature dropout \\
\midrule
$\mathcal I_X$ & 2,617/2,617 & 800/1,464 & 0/1,848 & 1,079/1,079 \\
$\mathcal I_{XF}$ & 2,617/2,617 & 685/1,464 & 6/1,848 & 1,057/1,079 \\
$\mathcal I_{Y_m}$ & 2,617/2,617 & 1,464/1,464 & 1,848/1,848 & 1,079/1,079 \\
$\mathcal I_{XFY}$ & 2,606/2,617 & 717/1,464 & 10/1,848 & 1,057/1,079 \\
$\mathcal I_{XFY}^{\star}$ & 0/2,617 & 0/1,464 & 0/1,848 & 0/1,079 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_policy_full.tex <==
\begin{table*}[!tbp]
\caption{Gate D: complete decision counts at the primary materiality threshold ($|\Delta_R|>0$; 7,008 material and 3,792 non-material intervened observations; 1,200 near-null synthetic controls). P0 serve-always, P1 union, P2 conformal, P3 sensor-coverage-complete relative to declared evidence dimensions and abstaining on missing coverage. Clean rows: 12,000 draws from evaluation pools disjoint from the calibration pools; resampled draws within a pool may overlap. The 1,200 exact-zero rows are used for $\mathcal I_{XFY}^{\star}$. B.\ hold/block: near-null controls held (statistical) or blocked (exact-reference violation). Integ.: non-material intervened observations held or blocked. Safe allow: clean, benign and non-material observations allowed. Interr.: non-material interruption rate, (false hold + false block + benign hold + benign block + integrity-only hold/block) over all non-material observations.}
\label{tab:s-policy-full}
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}llrrrrrrrrrrrr@{}}
\toprule
Regime & Pol. & Clean & F.\ hold & F.\ block & B.\ hold & B.\ block & Served & T.\ hold & T.\ block & Integ. & Imm.\ allow & Safe allow & Interr. \\
\midrule
$\mathcal I_X$ & P0 & 12,000 & 0 & 0 & 0 & 0 & 7,008 & 0 & 0 & 0 & 3,792 & 16,992 & 0.00 \\
$\mathcal I_X$ & P1 & 12,000 & 1,500 & 0 & 907 & 0 & 4,429 & 2,579 & 0 & 1,865 & 1,927 & 12,720 & 0.25 \\
$\mathcal I_X$ & P2 & 12,000 & 672 & 0 & 654 & 0 & 4,496 & 2,512 & 0 & 1,850 & 1,942 & 13,816 & 0.19 \\
$\mathcal I_X$ & P3 & 12,000 & 12,000 & 0 & 1,200 & 0 & 0 & 7,008 & 0 & 3,792 & 0 & 0 & 1.00 \\
\addlinespace[1pt]
$\mathcal I_{XF}$ & P0 & 12,000 & 0 & 0 & 0 & 0 & 7,008 & 0 & 0 & 0 & 3,792 & 16,992 & 0.00 \\
$\mathcal I_{XF}$ & P1 & 12,000 & 2,438 & 0 & 910 & 0 & 4,231 & 2,777 & 0 & 1,898 & 1,894 & 11,746 & 0.31 \\
$\mathcal I_{XF}$ & P2 & 12,000 & 695 & 0 & 622 & 0 & 4,365 & 2,643 & 0 & 1,830 & 1,962 & 13,845 & 0.19 \\
$\mathcal I_{XF}$ & P3 & 12,000 & 12,000 & 0 & 1,200 & 0 & 0 & 7,008 & 0 & 3,792 & 0 & 0 & 1.00 \\
\addlinespace[1pt]
$\mathcal I_{Y_m}$ & P0 & 12,000 & 0 & 0 & 0 & 0 & 7,008 & 0 & 0 & 0 & 3,792 & 16,992 & 0.00 \\
$\mathcal I_{Y_m}$ & P1 & 12,000 & 570 & 0 & 0 & 0 & 7,008 & 0 & 0 & 0 & 3,792 & 16,422 & 0.03 \\
$\mathcal I_{Y_m}$ & P2 & 12,000 & 570 & 0 & 0 & 0 & 7,008 & 0 & 0 & 0 & 3,792 & 16,422 & 0.03 \\
$\mathcal I_{Y_m}$ & P3 & 12,000 & 12,000 & 0 & 1,200 & 0 & 0 & 7,008 & 0 & 3,792 & 0 & 0 & 1.00 \\
\addlinespace[1pt]
$\mathcal I_{XFY}$ & P0 & 12,000 & 0 & 0 & 0 & 0 & 7,008 & 0 & 0 & 0 & 3,792 & 16,992 & 0.00 \\
$\mathcal I_{XFY}$ & P1 & 12,000 & 3,113 & 0 & 910 & 0 & 4,180 & 2,828 & 0 & 1,898 & 1,894 & 11,071 & 0.35 \\
$\mathcal I_{XFY}$ & P2 & 12,000 & 637 & 0 & 590 & 0 & 4,390 & 2,618 & 0 & 1,817 & 1,975 & 13,948 & 0.18 \\
$\mathcal I_{XFY}$ & P3 & 12,000 & 637 & 0 & 590 & 0 & 4,390 & 2,618 & 0 & 1,817 & 1,975 & 13,948 & 0.18 \\
\addlinespace[1pt]
$\mathcal I_{XFY}^{\star}$ & P0 & 1,200 & 0 & 0 & 0 & 0 & 7,008 & 0 & 0 & 0 & 3,792 & 6,192 & 0.00 \\
$\mathcal I_{XFY}^{\star}$ & P1 & 1,200 & 0 & 0 & 841 & 85 & 0 & 0 & 7,008 & 3,016 & 776 & 2,250 & 0.64 \\
$\mathcal I_{XFY}^{\star}$ & P2 & 1,200 & 0 & 0 & 544 & 85 & 0 & 0 & 7,008 & 2,944 & 848 & 2,619 & 0.58 \\
$\mathcal I_{XFY}^{\star}$ & P3 & 1,200 & 0 & 0 & 544 & 85 & 0 & 0 & 7,008 & 2,944 & 848 & 2,619 & 0.58 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_policy_rule_comparison.tex <==
\begin{table*}[!tbp]
\caption{Gate D: the risk-tolerant policy P2 under the superseded 1.2.0 family rule and under the adopted conformal rule, nominally calibrated under exchangeability, on identical observations ($|\Delta_R|>0$). The 1.2.0 columns reproduce the published 1.2.0 numbers and are retained for comparison only.}
\label{tab:s-policy-rule-comparison}
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
 & \multicolumn{4}{c}{1.2.0 rule (superseded)} & \multicolumn{4}{c}{Conformal rule (adopted)} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
Regime & Clean FPR & Benign & Served & Contain. & Clean FPR & Benign & Served & Contain. \\
\midrule
$\mathcal I_X$ & 0.061 & 0.58 & 4,494 & 0.36 & 0.056 & 0.55 & 4,496 & 0.36 \\
$\mathcal I_{XF}$ & 0.073 & 0.54 & 4,327 & 0.38 & 0.058 & 0.52 & 4,365 & 0.38 \\
$\mathcal I_{Y_m}$ & 0.048 & 0.00 & 7,008 & 0.00 & 0.048 & 0.00 & 7,008 & 0.00 \\
$\mathcal I_{XFY}$ & 0.079 & 0.53 & 4,322 & 0.38 & 0.053 & 0.49 & 4,390 & 0.37 \\
$\mathcal I_{XFY}^{\star}$ & 0.000 & 0.55 & 0 & 1.00 & 0.000 & 0.52 & 0 & 1.00 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_policy_tau.tex <==
\begin{table*}[!tbp]
\caption{Gate D: materially altered audit results served (containment in parentheses) under three materiality thresholds on $|\Delta_R|$; material observations 7,008, 3,802 and 1,870. The $\tau\to0^{+}$ column is a structural-sensitivity endpoint, whereas 0.02 and 0.05 are larger-effect sensitivity analyses. P1 union, P2 conformal.}
\label{tab:s-policy-tau}
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{@{}llrrr@{}}
\toprule
Regime & Pol. & $\tau=0^{+}$ & $\tau=0.02$ & $\tau=0.05$ \\
\midrule
$\mathcal I_X$ & P1 & 4,429 (0.37) & 2,128 (0.44) & 652 (0.65) \\
$\mathcal I_X$ & P2 & 4,496 (0.36) & 2,174 (0.43) & 680 (0.64) \\
$\mathcal I_{XF}$ & P1 & 4,231 (0.40) & 1,977 (0.48) & 566 (0.70) \\
$\mathcal I_{XF}$ & P2 & 4,365 (0.38) & 2,074 (0.45) & 629 (0.66) \\
$\mathcal I_{Y_m}$ & P1 & 7,008 (0.00) & 3,802 (0.00) & 1,870 (0.00) \\
$\mathcal I_{Y_m}$ & P2 & 7,008 (0.00) & 3,802 (0.00) & 1,870 (0.00) \\
$\mathcal I_{XFY}$ & P1 & 4,180 (0.40) & 1,926 (0.49) & 521 (0.72) \\
$\mathcal I_{XFY}$ & P2 & 4,390 (0.37) & 2,088 (0.45) & 629 (0.66) \\
$\mathcal I_{XFY}^{\star}$ & P1 & 0 (1.00) & 0 (1.00) & 0 (1.00) \\
$\mathcal I_{XFY}^{\star}$ & P2 & 0 (1.00) & 0 (1.00) & 0 (1.00) \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_v137_gate_f.tex <==
\begin{table*}[!tbp]
\caption{Corrected v1.3.7 Gate F on the unchanged null rows. Clean and near-null columns are response rates; the environment range is over the eight clean per-environment means. Re-split uses the same 30 frozen permutations; split construction uses the same fixed draw assignment. All are descriptive for the executed design except the conditional conformal counting statement under exchangeability.}
\label{tab:v137-gate-f}
\centering\scriptsize\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
Regime & Clean union & Clean asym. & Clean conf. & Env. conf. range & Near-null conf. & Re-split asym. & Re-split conf. & Split conf. \\
\midrule
$\mathcal I_X$ & 0.123 & 0.063 & 0.056 & 0.023--0.113 & 0.542 & 0.052 & 0.045 & 0.049 \\
$\mathcal I_{XF}$ & 0.201 & 0.074 & 0.059 & 0.024--0.130 & 0.502 & 0.058 & 0.042 & 0.036 \\
$\mathcal I_{Y_m}$ & 0.048 & 0.048 & 0.048 & 0.025--0.070 & 0.000 & 0.040 & 0.040 & 0.067 \\
$\mathcal I_{XFY}$ & 0.257 & 0.080 & 0.055 & 0.031--0.135 & 0.480 & 0.059 & 0.035 & 0.033 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_v137_label_geometry.tex <==
\begin{table*}[!t]
\caption{Label-side geometry sensitivity. Original uses $s(E,T_y(E))$; aligned uses $s(E,T_y(B))$ with clean comparator $s(E,B)$. Sensor columns are aligned means. Detection is on aligned material rows under $\IXFY$. Aggregate-blind rows preserve every declared label/confusion aggregate.}
\label{tab:v137-label-geometry}
\centering\footnotesize\setlength{\tabcolsep}{2.4pt}
\begin{tabular}{@{}lrrrrrrrrrrr@{}}
\toprule
Attack & $r$ & Mat. orig. & Mat. align. & Sep. & Blind & Label-$\Delta$ & Label-JSD & Conf.-L1 & Conf.-JSD & Family & Union \\
\midrule
prior-preserving & 0.02 & 262 & 283 & 283 & 317 & 0.038 & 0.001 & 0.125 & 0.005 & 24/283 & 118/283 \\
prior-preserving & 0.05 & 369 & 404 & 404 & 196 & 0.038 & 0.001 & 0.131 & 0.006 & 46/404 & 179/404 \\
prior-preserving & 0.10 & 428 & 421 & 421 & 179 & 0.038 & 0.001 & 0.146 & 0.007 & 74/421 & 200/421 \\
random & 0.02 & 521 & 516 & 563 & 37 & 0.039 & 0.001 & 0.127 & 0.005 & 54/516 & 186/516 \\
random & 0.05 & 499 & 548 & 599 & 1 & 0.040 & 0.001 & 0.137 & 0.006 & 65/548 & 244/548 \\
random & 0.10 & 538 & 528 & 566 & 34 & 0.040 & 0.001 & 0.149 & 0.007 & 80/528 & 256/528 \\
\midrule
\multicolumn{10}{l}{Pooled original frozen $\rightarrow$ geometry-aligned material response} & 11/2,617$\rightarrow$343/2,700 & 43/2,617$\rightarrow$1,183/2,700 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_v137_label_policy.tex <==
\begin{table*}[!t]
\caption{Label-only P2 sensitivity by geometry. Unsafe allow means a material altered audit result served in this frozen grid, not a deployed event rate. The trusted row uses the unchanged exact item-aligned checks.}
\label{tab:v137-label-policy}
\centering\footnotesize
\begin{tabular}{@{}llrrrrrr@{}}
\toprule
Geometry & Regime & $n$ & Material & Allow & Hold & Block & Unsafe allow \\
\midrule
original\_v136 & I\_X & 3600 & 2617 & 3600 & 0 & 0 & 2617 \\
original\_v136 & I\_XF & 3600 & 2617 & 3600 & 0 & 0 & 2617 \\
original\_v136 & I\_Ym & 3600 & 2617 & 3600 & 0 & 0 & 2617 \\
original\_v136 & I\_XFY & 3600 & 2617 & 3589 & 11 & 0 & 2606 \\
original\_v136 & I\_XFY\_trusted & 3600 & 2617 & 0 & 0 & 3600 & 0 \\
corrected\_original & I\_X & 3600 & 2617 & 3600 & 0 & 0 & 2617 \\
corrected\_original & I\_XF & 3600 & 2617 & 3600 & 0 & 0 & 2617 \\
corrected\_original & I\_Ym & 3600 & 2617 & 3600 & 0 & 0 & 2617 \\
corrected\_original & I\_XFY & 3600 & 2617 & 3589 & 11 & 0 & 2606 \\
corrected\_original & I\_XFY\_trusted & 3600 & 2617 & 0 & 0 & 3600 & 0 \\
aligned & I\_X & 3600 & 2700 & 3342 & 258 & 0 & 2506 \\
aligned & I\_XF & 3600 & 2700 & 3342 & 258 & 0 & 2509 \\
aligned & I\_Ym & 3600 & 2700 & 3258 & 342 & 0 & 2391 \\
aligned & I\_XFY & 3600 & 2700 & 3188 & 412 & 0 & 2357 \\
aligned & I\_XFY\_trusted & 3600 & 2700 & 0 & 0 & 3600 & 0 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_v137_mde.tex <==
\begin{table}[!tbp]
\caption{Descriptive lattice implication of the frozen confusion-profile L1 thresholds. Because the statistic lies on a $2/n$ lattice, the table gives the minimum net confusion-cell displacement needed to exceed each cell threshold. Relabelings can cancel in aggregate; these values are not minimum attack intensities or statistical-power guarantees.}
\label{tab:v137-mde}
\centering\scriptsize\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}rrrrr@{}}
\toprule
Batch $n$ & Cells & Threshold range & Net count range & Next L1 range \\
\midrule
256 & 6 & 0.171875--0.203125 & 23--27 & 0.179688--0.210938 \\
128 & 54 & 0.203125--0.281250 & 13--19 & 0.203125--0.296875 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/s_v137_policy_family.tex <==
\begin{table*}[!tbp]
\caption{Gate D after the JSD correction: materially altered audit results served / material observations by existing intervention mechanism under P2.}
\label{tab:s-policy-family}
\centering\scriptsize\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrrrr@{}}
\toprule
Regime & Evaluation-label & Sign flip & Mean shift / scaling & Feature dropout \\
\midrule
$\mathcal I_X$ & 2,617/2,617 & 800/1,464 & 0/1,848 & 1,079/1,079 \\
$\mathcal I_{XF}$ & 2,617/2,617 & 684/1,464 & 9/1,848 & 1,058/1,079 \\
$\mathcal I_{Y_m}$ & 2,617/2,617 & 1,464/1,464 & 1,848/1,848 & 1,079/1,079 \\
$\mathcal I_{XFY}$ & 2,606/2,617 & 716/1,464 & 14/1,848 & 1,058/1,079 \\
$\mathcal I_{XFY}^{\star}$ & 0/2,617 & 0/1,464 & 0/1,848 & 0/1,079 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_v137_policy_full.tex <==
\begin{table*}[!tbp]
\caption{Complete v1.3.7 Gate-D policy counts under the corrected JSD definition. These are deterministic decisions on the frozen rows, not deployed event rates. P3 coverage existence does not imply minimum statistical power.}
\label{tab:v137-policy-full}
\centering\scriptsize\setlength{\tabcolsep}{2.4pt}
\begin{tabular}{@{}llrrrrrrrr@{}}
\toprule
Regime & Policy & Clean $n$ & False act. & Near-null int. & Material & Allow & Hold & Block & Unsafe allow \\
\midrule
$\mathcal I_X$ & P0 & 12000 & 0 & 0 & 7008 & 10800 & 0 & 0 & 7008 \\
$\mathcal I_X$ & P1 union & 12000 & 1478 & 904 & 7008 & 6356 & 4444 & 0 & 4429 \\
$\mathcal I_X$ & P2 conf. & 12000 & 677 & 650 & 7008 & 6439 & 4361 & 0 & 4496 \\
$\mathcal I_X$ & P3 abst. & 12000 & 12000 & 1200 & 7008 & 0 & 10800 & 0 & 0 \\
\addlinespace[1pt]
$\mathcal I_{XF}$ & P0 & 12000 & 0 & 0 & 7008 & 10800 & 0 & 0 & 7008 \\
$\mathcal I_{XF}$ & P1 union & 12000 & 2417 & 905 & 7008 & 6127 & 4673 & 0 & 4233 \\
$\mathcal I_{XF}$ & P2 conf. & 12000 & 711 & 603 & 7008 & 6338 & 4462 & 0 & 4368 \\
$\mathcal I_{XF}$ & P3 abst. & 12000 & 12000 & 1200 & 7008 & 0 & 10800 & 0 & 0 \\
\addlinespace[1pt]
$\mathcal I_{Y_m}$ & P0 & 12000 & 0 & 0 & 7008 & 10800 & 0 & 0 & 7008 \\
$\mathcal I_{Y_m}$ & P1 union & 12000 & 570 & 0 & 7008 & 10800 & 0 & 0 & 7008 \\
$\mathcal I_{Y_m}$ & P2 conf. & 12000 & 570 & 0 & 7008 & 10800 & 0 & 0 & 7008 \\
$\mathcal I_{Y_m}$ & P3 abst. & 12000 & 12000 & 1200 & 7008 & 0 & 10800 & 0 & 0 \\
\addlinespace[1pt]
$\mathcal I_{XFY}$ & P0 & 12000 & 0 & 0 & 7008 & 10800 & 0 & 0 & 7008 \\
$\mathcal I_{XFY}$ & P1 union & 12000 & 3088 & 905 & 7008 & 6076 & 4724 & 0 & 4182 \\
$\mathcal I_{XFY}$ & P2 conf. & 12000 & 655 & 576 & 7008 & 6381 & 4419 & 0 & 4394 \\
$\mathcal I_{XFY}$ & P3 abst. & 12000 & 655 & 576 & 7008 & 6381 & 4419 & 0 & 4394 \\
\addlinespace[1pt]
$\mathcal I_{XFY}^{\star}$ & P0 & 1200 & 0 & 0 & 7008 & 10800 & 0 & 0 & 7008 \\
$\mathcal I_{XFY}^{\star}$ & P1 union & 1200 & 0 & 922 & 7008 & 776 & 1737 & 8287 & 0 \\
$\mathcal I_{XFY}^{\star}$ & P2 conf. & 1200 & 0 & 617 & 7008 & 857 & 1656 & 8287 & 0 \\
$\mathcal I_{XFY}^{\star}$ & P3 abst. & 1200 & 0 & 617 & 7008 & 857 & 1656 & 8287 & 0 \\
\addlinespace[1pt]
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_v137_policy_rule_comparison.tex <==
\begin{table*}[!tbp]
\caption{Gate D after the JSD correction: P2 under the superseded asymmetric rule and the adopted conformal rule on identical frozen observations. The comparison does not select or replace the primary rule.}
\label{tab:s-policy-rule-comparison}
\centering\scriptsize\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
 & \multicolumn{4}{c}{Asymmetric rule (superseded)} & \multicolumn{4}{c}{Conformal rule (adopted)} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
Regime & Clean FPR & Near-null & Served & Contain. & Clean FPR & Near-null & Served & Contain. \\
\midrule
$\mathcal I_X$ & 0.063 & 0.58 & 4,490 & 0.36 & 0.056 & 0.54 & 4,496 & 0.36 \\
$\mathcal I_{XF}$ & 0.074 & 0.53 & 4,329 & 0.38 & 0.059 & 0.50 & 4,368 & 0.38 \\
$\mathcal I_{Y_m}$ & 0.048 & 0.00 & 7,008 & 0.00 & 0.048 & 0.00 & 7,008 & 0.00 \\
$\mathcal I_{XFY}$ & 0.080 & 0.52 & 4,325 & 0.38 & 0.055 & 0.48 & 4,394 & 0.37 \\
$\mathcal I_{XFY}^{\star}$ & 0.000 & 0.55 & 0 & 1.00 & 0.000 & 0.51 & 0 & 1.00 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_v137_policy_tau.tex <==
\begin{table*}[!tbp]
\caption{Gate D after the JSD correction: materially altered audit results served (containment in parentheses) under the three frozen materiality thresholds. The thresholds select reporting endpoints, not attacks. P1 is union and P2 conformal.}
\label{tab:s-policy-tau}
\centering\scriptsize\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{@{}llrrr@{}}
\toprule
Regime & Pol. & $\tau=0^{+}$ & $\tau=0.02$ & $\tau=0.05$ \\
\midrule
$\mathcal I_X$ & P1 & 4,429 (0.37) & 2,128 (0.44) & 652 (0.65) \\
$\mathcal I_X$ & P2 & 4,496 (0.36) & 2,174 (0.43) & 680 (0.64) \\
$\mathcal I_{XF}$ & P1 & 4,233 (0.40) & 1,979 (0.48) & 566 (0.70) \\
$\mathcal I_{XF}$ & P2 & 4,368 (0.38) & 2,073 (0.45) & 628 (0.66) \\
$\mathcal I_{Y_m}$ & P1 & 7,008 (0.00) & 3,802 (0.00) & 1,870 (0.00) \\
$\mathcal I_{Y_m}$ & P2 & 7,008 (0.00) & 3,802 (0.00) & 1,870 (0.00) \\
$\mathcal I_{XFY}$ & P1 & 4,182 (0.40) & 1,928 (0.49) & 521 (0.72) \\
$\mathcal I_{XFY}$ & P2 & 4,394 (0.37) & 2,089 (0.45) & 628 (0.66) \\
$\mathcal I_{XFY}^{\star}$ & P1 & 0 (1.00) & 0 (1.00) & 0 (1.00) \\
$\mathcal I_{XFY}^{\star}$ & P2 & 0 (1.00) & 0 (1.00) & 0 (1.00) \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_v137_sensor_decomposition.tex <==
\begin{table*}[!b]
\caption{Original near-null controls: per-sensor decomposition by mechanism and strength. Each calibrated-sensor cell is mean response/firing percentage; KS-stat is descriptive only. Family columns are conformal fires.}
\label{tab:v137-decomp-1}
\centering\scriptsize\renewcommand{\arraystretch}{0.94}\setlength{\tabcolsep}{2.1pt}
\begin{tabular}{@{}lllrrrrrrrrr@{}}
\toprule
Class & Mechanism & Strength & F-JSD & MMD & KS-stat & KS-rej & S-JSD & $\Delta p$ & P-JSD & Fam. $\IX$ & Fam. $\IXF$ \\
\midrule
sham & tiny\_gaussian & 0.001 & 0.002/0\% & 0.000/0\% & 0.174 & 0.507/65\% & 0.007/0\% & 0.000/0\% & 0.000/0\% & 275/600 & 247/600 \\
sham & tiny\_scaling & 0.001 & 0.005/2\% & 0.001/0\% & 0.297 & 0.641/85\% & 0.035/12\% & 0.001/0\% & 0.000/0\% & 375/600 & 356/600 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[!t]
\caption{Original frozen feature interventions: per-sensor decomposition by mechanism and strength. Each calibrated-sensor cell is mean response/firing percentage; KS-stat is descriptive only. Family columns are conformal fires.}
\label{tab:v137-decomp-2}
\centering\scriptsize\renewcommand{\arraystretch}{0.94}\setlength{\tabcolsep}{2.1pt}
\begin{tabular}{@{}lllrrrrrrrrr@{}}
\toprule
Class & Mechanism & Strength & F-JSD & MMD & KS-stat & KS-rej & S-JSD & $\Delta p$ & P-JSD & Fam. $\IX$ & Fam. $\IXF$ \\
\midrule
corruption & sign\_flip & -- & 0.003/0\% & 0.026/12\% & 0.020 & 0.000/0\% & 0.024/0\% & 0.035/13\% & 0.003/13\% & 54/600 & 78/600 \\
corruption & sign\_flip & -- & 0.010/0\% & 0.117/53\% & 0.050 & 0.000/0\% & 0.065/23\% & 0.083/36\% & 0.011/38\% & 281/600 & 310/600 \\
corruption & sign\_flip & -- & 0.020/0\% & 0.193/76\% & 0.093 & 0.015/0\% & 0.124/72\% & 0.133/51\% & 0.025/51\% & 430/600 & 503/600 \\
covariate\_shift & mean\_shift & 0.020 & 0.065/53\% & 0.054/18\% & 0.533 & 0.959/100\% & 0.162/63\% & 0.013/3\% & 0.001/3\% & 600/600 & 584/600 \\
covariate\_shift & mean\_shift & 0.050 & 0.134/84\% & 0.122/34\% & 0.603 & 0.991/100\% & 0.253/79\% & 0.043/11\% & 0.010/12\% & 600/600 & 599/600 \\
covariate\_shift & mean\_shift & 0.100 & 0.187/90\% & 0.191/46\% & 0.623 & 0.994/100\% & 0.318/88\% & 0.089/22\% & 0.026/24\% & 600/600 & 600/600 \\
covariate\_shift & scaling\_drift & -- & 0.083/54\% & 0.087/25\% & 0.458 & 0.856/100\% & 0.225/63\% & 0.055/15\% & 0.014/16\% & 597/600 & 578/600 \\
covariate\_shift & scaling\_drift & -- & 0.152/72\% & 0.159/37\% & 0.520 & 0.890/100\% & 0.286/78\% & 0.133/30\% & 0.048/33\% & 599/600 & 587/600 \\
covariate\_shift & scaling\_drift & -- & 0.203/91\% & 0.241/55\% & 0.564 & 0.905/100\% & 0.330/89\% & 0.186/41\% & 0.076/43\% & 600/600 & 598/600 \\
pipeline & dropout & -- & 0.001/0\% & 0.000/0\% & 0.013 & 0.000/0\% & 0.008/0\% & 0.006/0\% & 0.000/0\% & 0/600 & 0/600 \\
pipeline & dropout & -- & 0.003/0\% & 0.000/0\% & 0.035 & 0.000/0\% & 0.023/0\% & 0.013/2\% & 0.000/2\% & 0/600 & 6/600 \\
pipeline & dropout & -- & 0.006/0\% & 0.000/0\% & 0.062 & 0.000/0\% & 0.038/4\% & 0.024/3\% & 0.001/4\% & 0/600 & 19/600 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[!t]
\caption{Original Gate A matched controls and adaptive variants: per-sensor decomposition by mechanism and strength. Each calibrated-sensor cell is mean response/firing percentage; KS-stat is descriptive only. Family columns are conformal fires.}
\label{tab:v137-decomp-3}
\centering\scriptsize\renewcommand{\arraystretch}{0.94}\setlength{\tabcolsep}{2.1pt}
\begin{tabular}{@{}lllrrrrrrrrr@{}}
\toprule
Class & Mechanism & Strength & F-JSD & MMD & KS-stat & KS-rej & S-JSD & $\Delta p$ & P-JSD & Fam. $\IX$ & Fam. $\IXF$ \\
\midrule
adaptive & mean\_shift & 0.020 & 0.014/1\% & 0.000/0\% & 0.045 & 0.029/1\% & 0.043/8\% & 0.004/0\% & 0.000/0\% & 4/600 & 31/600 \\
adaptive & mean\_shift & 0.050 & 0.027/8\% & 0.004/2\% & 0.065 & 0.070/4\% & 0.068/26\% & 0.008/0\% & 0.000/0\% & 50/600 & 135/600 \\
adaptive & mean\_shift & 0.100 & 0.039/35\% & 0.019/9\% & 0.082 & 0.117/9\% & 0.090/42\% & 0.018/3\% & 0.001/4\% & 215/600 & 298/600 \\
adaptive & mean\_shift & 0.250 & 0.074/80\% & 0.067/28\% & 0.133 & 0.287/41\% & 0.131/70\% & 0.048/16\% & 0.005/17\% & 484/600 & 498/600 \\
adaptive & mean\_shift & 0.500 & 0.085/88\% & 0.144/75\% & 0.153 & 0.354/58\% & 0.153/78\% & 0.081/34\% & 0.011/35\% & 530/600 & 537/600 \\
adaptive & scaling\_drift & 0.020 & 0.021/5\% & 0.003/0\% & 0.049 & 0.032/4\% & 0.064/26\% & 0.011/2\% & 0.001/2\% & 28/600 & 135/600 \\
adaptive & scaling\_drift & 0.050 & 0.041/32\% & 0.013/5\% & 0.069 & 0.077/8\% & 0.089/36\% & 0.029/10\% & 0.003/10\% & 173/600 & 254/600 \\
adaptive & scaling\_drift & 0.100 & 0.055/58\% & 0.036/17\% & 0.088 & 0.137/18\% & 0.106/49\% & 0.046/17\% & 0.006/17\% & 345/600 & 391/600 \\
adaptive & scaling\_drift & 0.250 & 0.074/75\% & 0.105/56\% & 0.125 & 0.260/41\% & 0.129/61\% & 0.075/30\% & 0.012/30\% & 451/600 & 479/600 \\
adaptive & scaling\_drift & 0.500 & 0.089/86\% & 0.185/82\% & 0.154 & 0.385/61\% & 0.141/67\% & 0.098/38\% & 0.018/38\% & 525/600 & 531/600 \\
control & mean\_shift & 0.020 & 0.065/53\% & 0.054/18\% & 0.533 & 0.959/100\% & 0.162/63\% & 0.013/3\% & 0.001/3\% & 600/600 & 584/600 \\
control & mean\_shift & 0.050 & 0.134/84\% & 0.122/34\% & 0.603 & 0.991/100\% & 0.253/79\% & 0.043/11\% & 0.010/12\% & 600/600 & 599/600 \\
control & mean\_shift & 0.100 & 0.187/90\% & 0.191/46\% & 0.623 & 0.994/100\% & 0.318/88\% & 0.089/22\% & 0.026/24\% & 600/600 & 600/600 \\
control & scaling\_drift & 0.020 & 0.083/54\% & 0.087/25\% & 0.458 & 0.856/100\% & 0.225/63\% & 0.055/15\% & 0.014/16\% & 597/600 & 578/600 \\
control & scaling\_drift & 0.050 & 0.152/72\% & 0.159/37\% & 0.520 & 0.890/100\% & 0.286/78\% & 0.133/30\% & 0.048/33\% & 599/600 & 587/600 \\
control & scaling\_drift & 0.100 & 0.203/91\% & 0.241/55\% & 0.564 & 0.905/100\% & 0.330/89\% & 0.186/41\% & 0.076/43\% & 600/600 & 598/600 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[!t]
\caption{Geometry-aligned feature sensitivity: per-sensor decomposition by mechanism and strength. Each calibrated-sensor cell is mean response/firing percentage; KS-stat is descriptive only. Family columns are conformal fires.}
\label{tab:v137-decomp-4}
\centering\scriptsize\renewcommand{\arraystretch}{0.94}\setlength{\tabcolsep}{2.1pt}
\begin{tabular}{@{}lllrrrrrrrrr@{}}
\toprule
Class & Mechanism & Strength & F-JSD & MMD & KS-stat & KS-rej & S-JSD & $\Delta p$ & P-JSD & Fam. $\IX$ & Fam. $\IXF$ \\
\midrule
adaptive & mean\_shift & 0.020 & 0.042/22\% & 0.032/11\% & 0.107 & 0.073/4\% & 0.078/27\% & 0.037/8\% & 0.002/9\% & 111/600 & 169/600 \\
adaptive & mean\_shift & 0.050 & 0.048/43\% & 0.039/14\% & 0.118 & 0.135/14\% & 0.094/45\% & 0.038/8\% & 0.002/9\% & 242/600 & 327/600 \\
adaptive & mean\_shift & 0.100 & 0.056/66\% & 0.055/28\% & 0.129 & 0.195/24\% & 0.109/62\% & 0.042/11\% & 0.003/12\% & 379/600 & 437/600 \\
adaptive & mean\_shift & 0.250 & 0.077/94\% & 0.096/50\% & 0.163 & 0.364/60\% & 0.139/80\% & 0.062/23\% & 0.006/26\% & 548/600 & 575/600 \\
adaptive & mean\_shift & 0.500 & 0.090/99\% & 0.160/80\% & 0.181 & 0.406/69\% & 0.159/86\% & 0.097/41\% & 0.013/42\% & 590/600 & 593/600 \\
adaptive & scaling\_drift & 0.020 & 0.046/34\% & 0.037/14\% & 0.111 & 0.097/10\% & 0.092/40\% & 0.039/10\% & 0.002/10\% & 184/600 & 285/600 \\
adaptive & scaling\_drift & 0.050 & 0.056/61\% & 0.052/24\% & 0.121 & 0.144/18\% & 0.108/55\% & 0.052/18\% & 0.004/20\% & 342/600 & 412/600 \\
adaptive & scaling\_drift & 0.100 & 0.065/76\% & 0.075/39\% & 0.132 & 0.206/32\% & 0.120/64\% & 0.065/24\% & 0.007/25\% & 461/600 & 486/600 \\
adaptive & scaling\_drift & 0.250 & 0.078/85\% & 0.132/70\% & 0.157 & 0.327/55\% & 0.137/72\% & 0.091/36\% & 0.013/36\% & 512/600 & 538/600 \\
adaptive & scaling\_drift & 0.500 & 0.091/91\% & 0.197/86\% & 0.179 & 0.433/69\% & 0.148/79\% & 0.111/43\% & 0.019/43\% & 550/600 & 559/600 \\
control & feature\_dropout & 0.020 & 0.039/7\% & 0.031/11\% & 0.102 & 0.042/3\% & 0.065/8\% & 0.038/8\% & 0.002/10\% & 41/600 & 38/600 \\
control & feature\_dropout & 0.050 & 0.039/9\% & 0.034/12\% & 0.111 & 0.087/8\% & 0.071/16\% & 0.042/11\% & 0.003/12\% & 52/600 & 84/600 \\
control & feature\_dropout & 0.100 & 0.040/10\% & 0.041/16\% & 0.128 & 0.182/23\% & 0.076/27\% & 0.048/17\% & 0.003/18\% & 131/600 & 182/600 \\
control & mean\_shift & 0.020 & 0.095/82\% & 0.083/31\% & 0.532 & 0.975/100\% & 0.188/77\% & 0.043/9\% & 0.003/10\% & 600/600 & 594/600 \\
control & mean\_shift & 0.050 & 0.157/93\% & 0.149/47\% & 0.603 & 0.992/100\% & 0.269/86\% & 0.070/18\% & 0.012/20\% & 600/600 & 600/600 \\
control & mean\_shift & 0.100 & 0.205/97\% & 0.217/62\% & 0.624 & 0.990/100\% & 0.329/93\% & 0.107/30\% & 0.028/32\% & 600/600 & 600/600 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[!t]
\caption{Geometry-aligned feature sensitivity: per-sensor decomposition by mechanism and strength. Each calibrated-sensor cell is mean response/firing percentage; KS-stat is descriptive only. Family columns are conformal fires.}
\label{tab:v137-decomp-5}
\centering\scriptsize\renewcommand{\arraystretch}{0.94}\setlength{\tabcolsep}{2.1pt}
\begin{tabular}{@{}lllrrrrrrrrr@{}}
\toprule
Class & Mechanism & Strength & F-JSD & MMD & KS-stat & KS-rej & S-JSD & $\Delta p$ & P-JSD & Fam. $\IX$ & Fam. $\IXF$ \\
\midrule
control & scaling\_drift & 0.020 & 0.108/71\% & 0.114/36\% & 0.461 & 0.857/100\% & 0.244/72\% & 0.080/20\% & 0.016/22\% & 600/600 & 584/600 \\
control & scaling\_drift & 0.050 & 0.167/90\% & 0.183/51\% & 0.521 & 0.895/100\% & 0.296/87\% & 0.152/36\% & 0.050/39\% & 600/600 & 595/600 \\
control & scaling\_drift & 0.100 & 0.212/95\% & 0.260/68\% & 0.564 & 0.916/100\% & 0.336/95\% & 0.200/44\% & 0.077/47\% & 600/600 & 600/600 \\
identity & identity & 0.000 & 0.039/7\% & 0.031/11\% & 0.100 & 0.038/2\% & 0.063/6\% & 0.036/7\% & 0.002/8\% & 43/600 & 43/600 \\
near\_null & tiny\_gaussian & 0.001 & 0.040/13\% & 0.031/11\% & 0.197 & 0.589/81\% & 0.066/10\% & 0.036/7\% & 0.002/8\% & 366/600 & 324/600 \\
near\_null & tiny\_scaling & 0.001 & 0.042/17\% & 0.032/12\% & 0.309 & 0.681/90\% & 0.088/29\% & 0.037/7\% & 0.002/8\% & 434/600 & 430/600 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[!t]
\caption{Gate-1 frozen design (response only; no family calibration): per-sensor decomposition by mechanism and strength. Each calibrated-sensor cell is mean response/firing percentage; KS-stat is descriptive only. Family columns are conformal fires.}
\label{tab:v137-decomp-6}
\centering\scriptsize\renewcommand{\arraystretch}{0.94}\setlength{\tabcolsep}{2.1pt}
\begin{tabular}{@{}lllrrrrrrrrr@{}}
\toprule
Class & Mechanism & Strength & F-JSD & MMD & KS-stat & KS-rej & S-JSD & $\Delta p$ & P-JSD & Fam. $\IX$ & Fam. $\IXF$ \\
\midrule
clean & unknown & -- & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & -- & -- \\
corruption & sign\_flip & -- & 0.003 & 0.020 & 0.018 & 0.000 & 0.027 & 0.045 & 0.002 & -- & -- \\
corruption & sign\_flip & -- & 0.009 & 0.107 & 0.046 & 0.000 & 0.073 & 0.103 & 0.009 & -- & -- \\
corruption & sign\_flip & -- & 0.022 & 0.192 & 0.094 & 0.010 & 0.142 & 0.171 & 0.023 & -- & -- \\
covariate\_shift & mean\_shift & 0.020 & 0.058 & 0.000 & 0.558 & 1.000 & 0.157 & 0.003 & 0.000 & -- & -- \\
covariate\_shift & mean\_shift & 0.050 & 0.127 & 0.001 & 0.604 & 1.000 & 0.234 & 0.005 & 0.000 & -- & -- \\
covariate\_shift & mean\_shift & 0.100 & 0.176 & 0.015 & 0.622 & 1.000 & 0.323 & 0.040 & 0.013 & -- & -- \\
covariate\_shift & scaling\_drift & -- & 0.098 & 0.001 & 0.486 & 0.849 & 0.323 & 0.018 & 0.003 & -- & -- \\
covariate\_shift & scaling\_drift & -- & 0.201 & 0.032 & 0.535 & 0.895 & 0.383 & 0.115 & 0.042 & -- & -- \\
covariate\_shift & scaling\_drift & -- & 0.267 & 0.116 & 0.578 & 0.923 & 0.421 & 0.304 & 0.117 & -- & -- \\
pipeline & dropout & -- & 0.001 & 0.000 & 0.014 & 0.000 & 0.009 & 0.003 & 0.000 & -- & -- \\
pipeline & dropout & -- & 0.002 & 0.000 & 0.034 & 0.000 & 0.025 & 0.006 & 0.000 & -- & -- \\
pipeline & dropout & -- & 0.004 & 0.000 & 0.060 & 0.000 & 0.041 & 0.014 & 0.000 & -- & -- \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_v137_without_ks.tex <==
\begin{table*}[!t]
\caption{Frozen-only descriptive ablation without the prespecified KS-reject component, Original frozen feature interventions. Cells give primary $\rightarrow$ without-KS conformal fire counts; this does not replace the primary family.}
\label{tab:v137-without-ks-1}
\centering\footnotesize\renewcommand{\arraystretch}{0.90}\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lllrrrr@{}}
\toprule
Class & Mechanism & Strength & $n$ & $\IX$ & $\IXF$ & $\IXFY$ \\
\midrule
corruption & sign\_flip & -- & 600 & 54$\rightarrow$54 & 78$\rightarrow$78 & 75$\rightarrow$75 \\
corruption & sign\_flip & -- & 600 & 281$\rightarrow$295 & 310$\rightarrow$315 & 283$\rightarrow$284 \\
corruption & sign\_flip & -- & 600 & 430$\rightarrow$435 & 503$\rightarrow$505 & 495$\rightarrow$496 \\
covariate\_shift & mean\_shift & 0.020 & 600 & 600$\rightarrow$342 & 584$\rightarrow$450 & 583$\rightarrow$441 \\
covariate\_shift & mean\_shift & 0.050 & 600 & 600$\rightarrow$518 & 599$\rightarrow$573 & 598$\rightarrow$571 \\
covariate\_shift & mean\_shift & 0.100 & 600 & 600$\rightarrow$542 & 600$\rightarrow$590 & 600$\rightarrow$588 \\
covariate\_shift & scaling\_drift & -- & 600 & 597$\rightarrow$339 & 578$\rightarrow$398 & 567$\rightarrow$396 \\
covariate\_shift & scaling\_drift & -- & 600 & 599$\rightarrow$452 & 587$\rightarrow$500 & 585$\rightarrow$497 \\
covariate\_shift & scaling\_drift & -- & 600 & 600$\rightarrow$563 & 598$\rightarrow$581 & 597$\rightarrow$577 \\
pipeline & dropout & -- & 600 & 0$\rightarrow$0 & 0$\rightarrow$0 & 0$\rightarrow$0 \\
pipeline & dropout & -- & 600 & 0$\rightarrow$0 & 6$\rightarrow$7 & 7$\rightarrow$7 \\
pipeline & dropout & -- & 600 & 0$\rightarrow$0 & 19$\rightarrow$20 & 18$\rightarrow$18 \\
target\_shift & label\_flip & -- & 600 & 0$\rightarrow$0 & 0$\rightarrow$0 & 0$\rightarrow$0 \\
target\_shift & label\_flip & -- & 600 & 0$\rightarrow$0 & 0$\rightarrow$0 & 0$\rightarrow$0 \\
target\_shift & label\_flip & -- & 600 & 0$\rightarrow$0 & 0$\rightarrow$0 & 4$\rightarrow$4 \\
target\_shift & label\_flip\_prior\_preserving & 0.020 & 600 & 0$\rightarrow$0 & 0$\rightarrow$0 & 0$\rightarrow$0 \\
target\_shift & label\_flip\_prior\_preserving & 0.050 & 600 & 0$\rightarrow$0 & 0$\rightarrow$0 & 0$\rightarrow$0 \\
target\_shift & label\_flip\_prior\_preserving & 0.100 & 600 & 0$\rightarrow$0 & 0$\rightarrow$0 & 7$\rightarrow$7 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[!t]
\caption{Frozen-only descriptive ablation without the prespecified KS-reject component, Geometry-aligned feature sensitivity. Cells give primary $\rightarrow$ without-KS conformal fire counts; this does not replace the primary family.}
\label{tab:v137-without-ks-2}
\centering\footnotesize\renewcommand{\arraystretch}{0.90}\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lllrrrr@{}}
\toprule
Class & Mechanism & Strength & $n$ & $\IX$ & $\IXF$ & $\IXFY$ \\
\midrule
adaptive & mean\_shift & 0.020 & 600 & 111$\rightarrow$115 & 169$\rightarrow$171 & 167$\rightarrow$171 \\
adaptive & mean\_shift & 0.050 & 600 & 242$\rightarrow$245 & 327$\rightarrow$325 & 312$\rightarrow$320 \\
adaptive & mean\_shift & 0.100 & 600 & 379$\rightarrow$384 & 437$\rightarrow$437 & 417$\rightarrow$428 \\
adaptive & mean\_shift & 0.250 & 600 & 548$\rightarrow$556 & 575$\rightarrow$577 & 570$\rightarrow$571 \\
adaptive & mean\_shift & 0.500 & 600 & 590$\rightarrow$591 & 593$\rightarrow$592 & 586$\rightarrow$590 \\
adaptive & scaling\_drift & 0.020 & 600 & 184$\rightarrow$188 & 285$\rightarrow$285 & 265$\rightarrow$271 \\
adaptive & scaling\_drift & 0.050 & 600 & 342$\rightarrow$349 & 412$\rightarrow$416 & 404$\rightarrow$408 \\
adaptive & scaling\_drift & 0.100 & 600 & 461$\rightarrow$460 & 486$\rightarrow$485 & 480$\rightarrow$481 \\
adaptive & scaling\_drift & 0.250 & 600 & 512$\rightarrow$517 & 538$\rightarrow$539 & 534$\rightarrow$535 \\
adaptive & scaling\_drift & 0.500 & 600 & 550$\rightarrow$556 & 559$\rightarrow$561 & 551$\rightarrow$558 \\
control & feature\_dropout & 0.020 & 600 & 41$\rightarrow$44 & 38$\rightarrow$41 & 42$\rightarrow$43 \\
control & feature\_dropout & 0.050 & 600 & 52$\rightarrow$56 & 84$\rightarrow$83 & 80$\rightarrow$85 \\
control & feature\_dropout & 0.100 & 600 & 131$\rightarrow$94 & 182$\rightarrow$160 & 156$\rightarrow$149 \\
control & mean\_shift & 0.020 & 600 & 600$\rightarrow$506 & 594$\rightarrow$550 & 592$\rightarrow$545 \\
control & mean\_shift & 0.050 & 600 & 600$\rightarrow$573 & 600$\rightarrow$592 & 600$\rightarrow$592 \\
control & mean\_shift & 0.100 & 600 & 600$\rightarrow$588 & 600$\rightarrow$598 & 600$\rightarrow$598 \\
control & scaling\_drift & 0.020 & 600 & 600$\rightarrow$444 & 584$\rightarrow$485 & 576$\rightarrow$477 \\
control & scaling\_drift & 0.050 & 600 & 600$\rightarrow$564 & 595$\rightarrow$579 & 592$\rightarrow$574 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[!t]
\caption{Frozen-only descriptive ablation without the prespecified KS-reject component, Geometry-aligned feature sensitivity. Cells give primary $\rightarrow$ without-KS conformal fire counts; this does not replace the primary family.}
\label{tab:v137-without-ks-3}
\centering\footnotesize\renewcommand{\arraystretch}{0.90}\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lllrrrr@{}}
\toprule
Class & Mechanism & Strength & $n$ & $\IX$ & $\IXF$ & $\IXFY$ \\
\midrule
control & scaling\_drift & 0.100 & 600 & 600$\rightarrow$590 & 600$\rightarrow$597 & 600$\rightarrow$596 \\
identity & identity & 0.000 & 600 & 43$\rightarrow$47 & 43$\rightarrow$44 & 48$\rightarrow$50 \\
near\_null & tiny\_gaussian & 0.001 & 600 & 366$\rightarrow$67 & 324$\rightarrow$70 & 313$\rightarrow$70 \\
near\_null & tiny\_scaling & 0.001 & 600 & 434$\rightarrow$109 & 430$\rightarrow$175 & 414$\rightarrow$177 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[!t]
\caption{Frozen-only descriptive ablation without the prespecified KS-reject component, Original Gate A matched controls and adaptive variants. Cells give primary $\rightarrow$ without-KS conformal fire counts; this does not replace the primary family.}
\label{tab:v137-without-ks-4}
\centering\footnotesize\renewcommand{\arraystretch}{0.90}\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lllrrrr@{}}
\toprule
Class & Mechanism & Strength & $n$ & $\IX$ & $\IXF$ & $\IXFY$ \\
\midrule
adaptive & mean\_shift & 0.020 & 600 & 4$\rightarrow$4 & 31$\rightarrow$31 & 27$\rightarrow$27 \\
adaptive & mean\_shift & 0.050 & 600 & 50$\rightarrow$49 & 135$\rightarrow$138 & 127$\rightarrow$126 \\
adaptive & mean\_shift & 0.100 & 600 & 215$\rightarrow$219 & 298$\rightarrow$301 & 280$\rightarrow$282 \\
adaptive & mean\_shift & 0.250 & 600 & 484$\rightarrow$486 & 498$\rightarrow$501 & 486$\rightarrow$493 \\
adaptive & mean\_shift & 0.500 & 600 & 530$\rightarrow$530 & 537$\rightarrow$538 & 530$\rightarrow$536 \\
adaptive & scaling\_drift & 0.020 & 600 & 28$\rightarrow$26 & 135$\rightarrow$136 & 129$\rightarrow$129 \\
adaptive & scaling\_drift & 0.050 & 600 & 173$\rightarrow$180 & 254$\rightarrow$254 & 237$\rightarrow$242 \\
adaptive & scaling\_drift & 0.100 & 600 & 345$\rightarrow$337 & 391$\rightarrow$391 & 378$\rightarrow$383 \\
adaptive & scaling\_drift & 0.250 & 600 & 451$\rightarrow$453 & 479$\rightarrow$480 & 467$\rightarrow$472 \\
adaptive & scaling\_drift & 0.500 & 600 & 525$\rightarrow$529 & 531$\rightarrow$535 & 521$\rightarrow$524 \\
control & mean\_shift & 0.020 & 600 & 600$\rightarrow$342 & 584$\rightarrow$450 & 583$\rightarrow$441 \\
control & mean\_shift & 0.050 & 600 & 600$\rightarrow$518 & 599$\rightarrow$573 & 598$\rightarrow$571 \\
control & mean\_shift & 0.100 & 600 & 600$\rightarrow$542 & 600$\rightarrow$590 & 600$\rightarrow$588 \\
control & scaling\_drift & 0.020 & 600 & 597$\rightarrow$339 & 578$\rightarrow$398 & 567$\rightarrow$396 \\
control & scaling\_drift & 0.050 & 600 & 599$\rightarrow$452 & 587$\rightarrow$500 & 585$\rightarrow$497 \\
control & scaling\_drift & 0.100 & 600 & 600$\rightarrow$563 & 598$\rightarrow$581 & 597$\rightarrow$577 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[!t]
\caption{Frozen-only descriptive ablation without the prespecified KS-reject component, Geometry-aligned label sensitivity and original near-null controls. Cells give primary $\rightarrow$ without-KS conformal fire counts; this does not replace the primary family.}
\label{tab:v137-without-ks-5}
\centering\footnotesize\renewcommand{\arraystretch}{0.90}\setlength{\tabcolsep}{4pt}
\begin{tabular}{@{}lllrrrr@{}}
\toprule
Class & Mechanism & Strength & $n$ & $\IX$ & $\IXF$ & $\IXFY$ \\
\midrule
label & label\_flip & 0.020 & 600 & 43$\rightarrow$47 & 43$\rightarrow$44 & 64$\rightarrow$66 \\
label & label\_flip & 0.050 & 600 & 43$\rightarrow$47 & 43$\rightarrow$44 & 69$\rightarrow$71 \\
label & label\_flip & 0.100 & 600 & 43$\rightarrow$47 & 43$\rightarrow$44 & 84$\rightarrow$86 \\
label & label\_flip\_prior\_preserving & 0.020 & 600 & 43$\rightarrow$47 & 43$\rightarrow$44 & 48$\rightarrow$50 \\
label & label\_flip\_prior\_preserving & 0.050 & 600 & 43$\rightarrow$47 & 43$\rightarrow$44 & 55$\rightarrow$57 \\
label & label\_flip\_prior\_preserving & 0.100 & 600 & 43$\rightarrow$47 & 43$\rightarrow$44 & 92$\rightarrow$95 \\
sham & tiny\_gaussian & 0.001 & 600 & 275$\rightarrow$0 & 247$\rightarrow$1 & 243$\rightarrow$1 \\
sham & tiny\_scaling & 0.001 & 600 & 375$\rightarrow$10 & 356$\rightarrow$63 & 333$\rightarrow$61 \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/s_witnesses.tex <==
\begin{table}[!tbp]
\caption{Counterexample witnesses realised in the frozen expansion (count / denominator). W1--W4 are evaluation-label rows, W5--W6 feature-side rows, W7 all intervened rows, W8 material label rows; W9 and W10 count the label rows that a trusted aggregate reference, respectively only an item-aligned reference, detects (Corollary~3).}
\label{tab:s-witnesses}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{tabularx}{\columnwidth}{@{}l>{\raggedright\arraybackslash}Xr@{}}
\toprule
ID & Property & Count \\
\midrule
W1 & identity change without joint-outcome or conclusion change & 808 / 3,600 \\
W2 & conclusion change without model-output change & 2,617 / 3,600 \\
W3 & marginal invariance with conclusion change & 1,059 / 1,800 \\
W4 & confusion-profile change without conclusion change & 175 / 3,600 \\
W5 & model-output change without conclusion change & 296 / 7,200 \\
W6 & representation change without output change & 2,513 / 7,200 \\
W7 & apparent improvement under intervention & 1,534 / 10,800 \\
W8 & material conclusion change always changes the confusion profile (label path) & 2,617 / 2,617 \\
W9 & label rows detectable by a trusted aggregate (confusion-matrix) reference of the same batch & 2,792 / 3,600 \\
W10 & label rows detectable only by an item-aligned reference & 808 / 3,600 \\
\bottomrule
\end{tabularx}
\end{table}

